Enhancing Supervised Visualization through Autoencoder and Random Forest Proximities for Out-of-Sample Extension

The value of supervised dimensionality reduction lies in its ability to uncover meaningful connections between data features and labels. Common dimensionality reduction methods embed a set of fixed, latent points, but are not capable of generalizing to an unseen test set. In this paper, we provide an out-of-sample extension method for the random forest-based supervised dimensionality reduction method, RF-PHATE, combining information learned from the random forest model with the function-learning capabilities of autoencoders. Through quantitative assessment of various autoencoder architectures, we identify that networks that reconstruct random forest proximities are more robust for the embedding extension problem. Furthermore, by leveraging proximity-based prototypes, we achieve a 40% reduction in training time without compromising extension quality. Our method does not require label information for out-of-sample points, thus serving as a semi-supervised method, and can achieve consistent quality using only 10% of the training data.

==> ida_reviews.tex <==
TODO Regarding Reviews:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Add summary of results and info about experiments in the abstract.
Add separate related works section (may be infeasible due to shortened MLSP paper)
Double check all acronyms.
Check naming conventions listed in paper and in figures for consistency.
Check statistical significance of results from experiments.
Add baselines, introduce performance metrics, and structure the experiments section better
Share the code of the project via Github. (Check MLSP guidelines).
Improvement in the clarity of the experiments and terms, as well as the inclusion of a broader literature review, as recommended by the reviewers.
Literature review recommendations may be less important due to spacing issues.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Reviewer 1:

The paper proposes an out-of-sample extension method for the random forest-based supervised dimensionality reduction. The approach is based on a combination of random forest and autoencoders. The method is tested on 26 datasets,

In general, the methods section is nicely written and easy to follow. The authors present novel contributions, including a regularisation approach for autoencoders, an extension of random forest proximity measures and overall architecture to combine methods. The readability of the paper decreases significantly in the experiments section. The purpose of experiments, baselines, and performance metrics are not sufficiently introduced.

The main issue I see lies in the experiments section. There are no objective comparisons against well-known/state-of-the-art baselines. The comparison presented seems to be more of an ablation study. In the abstract, the main motivation is the weakness of other methods in out-of-sample generalisation. It is not clear how this is achieved with this method compared to the other methods.


- Please add a summary of results and information about experiments in the abstract.
- I strongly suggest adding a separate related work section
- Various acronyms are not introduced at all, and some are not properly introduced in the text (e.g., the acronym OOSE is only introduced in the conclusion while it has been used before in the text.). I suggest not to use an acronym for this term.
- In Fig1, it would be best to use all the steps' names (1-5). Currently, the text's naming is inconsistent with what you present in the figure.
- Please show the significance of the results in Tables using a statistical test.
- Please add baselines, introduce performance metrics, and structure the experiments section better


Reviewer 3:

This paper considers the problem of lacking a function for out-of-sample extension which is solved by combining Random Forest and Auto-encoder.

The main ideas of the paper are not novel or represent incremental advances. However, this paper is well-written and the experimental evaluation is adequate, and the results convincingly support the main claims.

Reviewer 5:

In the context of data dimensionality reduction, this paper proposes an extension of RF-PHATE: a Random Forest supervised dimensionality reduction method. The extended method combines information learned from random forest model with the function learning capabilities of autoencoders to effectively visualize out-of-sample data points.
This is an interesting contribution to the field of supervised dimensionality reduction, which complements and improves the exiting methods in that field. I expect promising applications of the proposed method.
The paper is well structured, starting with a good introduction where the context is outlined, the problem highlighted and well positioned within the literature, the contribution is clearly defined.
In the methodology, in addition to formal definitions of the method components (autoencoders and random forest proximities, PHATE, and Out-of-Sample Extension), the RF-PROX-RECON-PRO (random forest-proximity reconstruction) architecture and model is well described and explained supported by a schematic figure.
In the experiments section, the authors used 26 datasets and 10 repetitions which is a good number to assess their model performance compared to other models. The results are promising and advantageous for large datasets.
Minor improvements:
- Check abbreviations. Some abbreviations were used for the first time but not explained what they refer to. E.g. OOSE: Out of Sample Extension.
- For the purpose of open science, I wonder if the authors would like to share the code of the project via Github.


Meta-Reviewer 2:

The paper presents a dimensionality reduction approach that combines auto-encoders with random forest for meaningful data visualization. The paper is well-structured, and the overall approach, problem statement, and the empirical study are promising and somewhat novel. However, there is room for improvement in the clarity of the experiments and terms, as well as the inclusion of a broader literature review, as recommended by the reviewers. Overall, I'm leaning toward accepting the paper.

==> references_old.tex <==
@article {rhodes2024gaining,
    author = {Jake S. Rhodes and Adrien Aumon and Sacha Morin and Marc Girard and Catherine Larochelle and Elsa Brunet-Ratnasingham and Am{\'e}lie Pagliuzza and Lorie Marchitto and Wei Zhang and Adele Cutler and Francois Grand{\textquoteright}Maison and Anhong Zhou and Andr{\'e}s Finzi and Nicolas Chomont and Daniel E. Kaufmann and Stephanie Zandee and Alexandre Prat and Guy Wolf and Kevin R. Moon},
    title = {Gaining Biological Insights through Supervised Data Visualization},
    elocation-id = {2023.11.22.568384},
    year = {2024},
    doi = {10.1101/2023.11.22.568384},
    publisher = {Cold Spring Harbor Laboratory},
    abstract = {Dimensionality reduction-based data visualization is pivotal in comprehending complex biological data. The most common methods, such as PHATE, t-SNE, and UMAP, are unsupervised and therefore reflect the dominant structure in the data, which may be independent of expert-provided labels. Here we introduce a supervised data visualization method called RF-PHATE, which integrates expert knowledge for further exploration of the data. RF-PHATE leverages random forests to capture intricate featurelabel relationships. Extracting information from the forest, RF-PHATE generates low-dimensional visualizations that highlight relevant data relationships while disregarding extraneous features. This approach scales to large datasets and applies to classification and regression. We illustrate RF-PHATE{\textquoteright}s prowess through three case studies. In a multiple sclerosis study using longitudinal clinical and imaging data, RF-PHATE unveils a sub-group of patients with non-benign relapsingremitting Multiple Sclerosis, demonstrating its aptitude for time-series data. In the context of Raman spectral data, RF-PHATE effectively showcases the impact of antioxidants on diesel exhaust-exposed lung cells, highlighting its proficiency in noisy environments. Furthermore, RF-PHATE aligns established geometric structures with COVID-19 patient outcomes, enriching interpretability in a hierarchical manner. RF-PHATE bridges expert insights and visualizations, promising knowledge generation. Its adaptability, scalability, and noise tolerance underscore its potential for widespread adoption.Competing Interest StatementThe authors have declared no competing interest.},
    URL = {https://www.biorxiv.org/content/early/2024/01/21/2023.11.22.568384},
    eprint = {https://www.biorxiv.org/content/early/2024/01/21/2023.11.22.568384.full.pdf},
    journal = {bioRxiv}
}


@INPROCEEDINGS{tsuge2001nmfdim,
  author={Tsuge, S. and Shishibori, M. and Kuroiwa, S. and Kita, K.},
  booktitle={2001 IEEE International Conference on Systems, Man and Cybernetics. e-Systems and e-Man for Cybernetics in Cyberspace (Cat.No.01CH37236)}, 
  title={Dimensionality reduction using non-negative matrix factorization for information retrieval}, 
  year={2001},
  volume={2},
  number={},
  pages={960-965 vol.2},
  doi={10.1109/ICSMC.2001.973042}}


@Article{Haghverdi2016dpt,
author={Haghverdi, L.
and B{\"u}ttner, M.
and Wolf, F. A.
and Buettner, F.
and Theis, F. J.},
title={Diffusion pseudotime robustly reconstructs lineage branching},
journal={Nature Methods},
year={2016},
month={Oct},
day={01},
volume={13},
number={10},
pages={845-848},
abstract={Diffusion pseudotime (DPT) enables robust and scalable inference of cellular trajectories, branching events, metastable states and underlying gene dynamics from snapshot single-cell gene expression data.},
issn={1548-7105},
doi={10.1038/nmeth.3971},
url={https://doi.org/10.1038/nmeth.3971}
}

@article{kuchroo2022multiscale,
  title={Multiscale PHATE identifies multimodal signatures of COVID-19},
  author={Kuchroo, M. and Huang, J. and Wong, P. and Grenier, J. and Shung, D. and Tong, A. and Lucas, C. and Klein, J. and Burkhardt, D. B and Gigante, S. and others},
  journal={Nature biotechnology},
  volume={40},
  number={5},
  pages={681--691},
  year={2022},
  publisher={Nature Publishing Group US New York}
}

@article{malepathirana2022song,
  title={Dimensionality reduction for visualizing high-dimensional biological data},
  author={Malepathirana, T. and Senanayake, D. and Vidanaarachchi, R. and Gautam, V. and Halgamuge, S.},
  journal={Biosystems},
  volume={220},
  pages={104749},
  year={2022},
  publisher={Elsevier}
}

@article{milovsevic2022aquatic,
  title={The application of Uniform Manifold Approximation and Projection (UMAP) for unconstrained ordination and classification of biological indicators in aquatic ecology},
  author={Milo{\v{s}}evi{\'c}, Djuradj and Medeiros, Andrew S and Piperac, Milica Stojkovi{\'c} and Cvijanovi{\'c}, Du{\v{s}}anka and Soininen, Janne and Milosavljevi{\'c}, Aleksandar and Predi{\'c}, Bratislav},
  journal={Science of The Total Environment},
  volume={815},
  pages={152365},
  year={2022},
  publisher={Elsevier}
}

@article{jiang2022bearing,
  title={Fault diagnosis for rolling bearing using a hybrid hierarchical method based on scale-variable dispersion entropy and parametric t-SNE algorithm},
  author={Jiang, Wei and Xu, Yanhe and Chen, Zhong and Zhang, Nan and Zhou, Jianzhong},
  journal={Measurement},
  volume={191},
  pages={110843},
  year={2022},
  publisher={Elsevier}
}





@Article{Breiman2001randomforests,
    author={L. Breiman},
    title={Random Forests},
    journal={Mach. Learn.},
    year={2001},
    month={Oct.},
    day={01},
    volume={45},
    number={1},
    pages={5-32},
    abstract={Random forests are a combination of tree predictors such that each tree depends on the values of a random vector sampled independently and with the same distribution for all trees in the forest. The generalization error for forests converges a.s. to a limit as the number of trees in the forest becomes large. The generalization error of a forest of tree classifiers depends on the strength of the individual trees in the forest and the correlation between them. Using a random selection of features to split each node yields error rates that compare favorably to Adaboost (Y. Freund {\&} R. Schapire, Machine Learning: Proceedings of the Thirteenth International Conference, ***, 148--156), but are more robust with respect to noise. Internal estimates monitor error, strength, and correlation and these are used to show the response to increasing the number of features used in the splitting. Internal estimates are also used to measure variable importance. These ideas are also applicable to regression.},
    issn={1573-0565},
    doi={10.1023/A:1010933404324},
    url={http://doi.org/10.1023/A:1010933404324}
}

% TODO:
@misc{BreimanRandomForest:Online,
    author = {Breiman, L. and Cutler, A.},
    title = {Random Forests},
    howpublished = {\url{https://www.stat.berkeley.edu/~breiman/RandomForests/}},
    note = {Accessed: 11/13/2023}
    }

@article{lin2006adaptiveNN,
 ISSN = {01621459},
 abstract = {In this article we study random forests through their connection with a new framework of adaptive nearest-neighbor methods. We introduce a concept of potential nearest neighbors (k-PNNs) and show that random forests can be viewed as adaptively weighted k-PNN methods. Various aspects of random forests can be studied from this perspective. We study the effect of terminal node sizes on the prediction accuracy of random forests. We further show that random forests with adaptive splitting schemes assign weights to k-PNNs in a desirable way: for the estimation at a given target point, these random forests assign voting weights to the k-PNNs of the target point according to the local importance of different input variables. We propose a new simple splitting scheme that achieves desirable adaptivity in a straightforward fashion. This simple scheme can be combined with existing algorithms. The resulting algorithm is computationally faster and gives comparable results. Other possible aspects of random forests, such as using linear combinations in splitting, are also discussed. Simulations and real datasets are used to illustrate the results.},
 author = {Yi Lin and Yongho Jeon},
 journal = {J. Am. Stat. Assoc.},
 number = {474},
 pages = {578--590},
 publisher = {[American Statistical Association, Taylor & Francis, Ltd.]},
 title = {Random Forests and Adaptive Nearest Neighbors},
 volume = {101},
 year = {2006},
 url = {https://doi.org/10.1198/016214505000001230}
}

@article{Zhou2010GeneSU,
  title={Gene Selection Using Random Forest and Proximity Differences Criterion on DNA Microarray Data},
  author={Q. Zhou and W. Hong and L. Luo and F. Yang},
  journal={J. Convergence Inf. Technol.},
  year={2010},
  volume={5},
  pages={161-170},
}

@InProceedings{gray2011dementia,
    author="Gray, K. R.
    and Aljabar, P.
    and Heckemann, R. A.
    and Hammers, A.
    and Rueckert, D.",
    editor="Suzuki, Kenji
    and Wang, Fei
    and Shen, D.
    and Yan, P.",
    title="Random Forest-Based Manifold Learning for Classification of Imaging Data in Dementia",
    booktitle="Machine Learning in Medical Imaging",
    year="2011",
    publisher="Springer",
    address="Berlin, Heidelberg",
    pages="159--166",
    abstract="Neurodegenerative disorders are characterized by changes in multiple biomarkers, which may provide complementary information for diagnosis and prognosis. We present a framework in which proximities derived from random forests are used to learn a low-dimensional manifold from labelled training data and then to infer the clinical labels of test data mapped to this space. The proposed method facilitates the combination of embeddings from multiple datasets, resulting in the generation of a joint embedding that simultaneously encodes information about all the available features. It is possible to combine different types of data without additional processing, and we demonstrate this key feature by application to voxel-based FDG-PET and region-based MR imaging data from the ADNI study. Classification based on the joint embedding coordinates out-performs classification based on either modality alone. Results are impressive compared with other state-of-the-art machine learning techniques applied to multi-modality imaging data.",
    isbn="978-3-642-24319-6"
}

% TODO:
@inproceedings{seoane2014geneannotation,
  title = {A Random Forest proximity matrix as a new measure for gene annotation},
  author = {José A. Seoane and Ian N. M. Day and Juan P. Casas and Colin Campbell and Tom R. Gaunt},
  year = {2014},
  researchr = {https://researchr.org/publication/SeoaneDCCG14},
  booktitle = {22th European Symposium on Artificial Neural Networks, ESANN 2014, Bruges, Belgium, April 23-25, 2014},
}


@Article{Zhao2016propensity,
    author={Zhao, P.
    and Su, X.
    and Ge, T.
    and Fan, J.},
    title={Propensity score and proximity matching using random forest},
    journal={Contemp. Clin. Trials},
    year={2016},
    month={Mar},
    edition={2015/12/17},
    volume={47},
    pages={85-92},
    keywords={Matching; Observational study; Propensity score; Proximity; Random forest; Adult; Aged; Body Mass Index; Case-Control Studies; Data Interpretation, Statistical; Databases, Factual; Female; Humans; Male; Middle Aged; Nutrition Surveys; Obesity/*epidemiology; *Propensity Score; Smoking/*epidemiology; Statistics as Topic; United States/epidemiology},
    abstract={In order to derive unbiased inference from observational data, matching methods are often applied to produce balanced treatment and control groups in terms of all background variables. Propensity score has been a key component in this research area. However, propensity score based matching methods in the literature have several limitations, such as model mis-specifications, categorical variables with more than two levels, difficulties in handling missing data, and nonlinear relationships. Random forest, averaging outcomes from many decision trees, is nonparametric in nature, straightforward to use, and capable of solving these issues. More importantly, the precision afforded by random forest (Caruana et al., 2008) may provide us with a more accurate and less model dependent estimate of the propensity score. In addition, the proximity matrix, a by-product of the random forest, may naturally serve as a distance measure between observations that can be used in matching. The proposed random forest based matching methods are applied to data from the National Health and Nutrition Examination Survey (NHANES). Our results show that the proposed methods can produce well balanced treatment and control groups. An illustration is also provided that the methods can effectively deal with missing data in covariates.},
    issn={1559-2030},
    doi={10.1016/j.cct.2015.12.012},
    language={eng},
    url = {http://doi.org/10.1016/j.cct.2015.12.012}
}

@misc{whitmore2018explicating,
      title={Explicating feature contribution using Random Forest proximity distances}, 
      author={L. S. Whitmore and A. George and C. M. Hudson},
      year={2018},
      eprint={1807.06572},
      archivePrefix={arXiv},
      primaryClass={stat.ML},
      url = {https://arxiv.org/abs/1807.06572}
}

@article{ishwaran2007vimp,
    author = "Ishwaran, H.",
    doi = "10.1214/07-EJS039",
    fjournal = "Electronic Journal of Statistics",
    journal = "Electron. J. Stat.",
    pages = "519--537",
    publisher = "The Institute of Mathematical Statistics and the Bernoulli Society",
    title = "Variable importance in binary regression trees and forests",
    volume = "1",
    year = "2007"
}

@Article{Strobl2008conditionalVIMP,
    author={Strobl, C.
    and Boulesteix, A.
    and Kneib, T.
    and Augustin, T.
    and Zeileis, A.},
    title={Conditional variable importance for random forests},
    journal={BMC Bioinf.},
    year={2008},
    month={Jul},
    day={11},
    volume={9},
    number={1},
    pages={307},
    abstract={Random forests are becoming increasingly popular in many scientific fields because they can cope with "small n large p" problems, complex interactions and even highly correlated predictor variables. Their variable importance measures have recently been suggested as screening tools for, e.g., gene expression studies. However, these variable importance measures show a bias towards correlated predictor variables.},
    issn={1471-2105},
    doi={10.1186/1471-2105-9-307}
}

@Article{Nicodemus2010permImpBehaviour,
    author={Nicodemus, K. K.
    and Malley, J. D.
    and Strobl, C.
    and Ziegler, A.},
    title={The behaviour of random forest permutation-based variable importance measures under predictor correlation},
    journal={BMC Bioinf.},
    year={2010},
    month={Feb},
    day={27},
    volume={11},
    number={1},
    pages={110},
    abstract={Random forests (RF) have been increasingly used in applications such as genome-wide association and microarray studies where predictor correlation is frequently observed. Recent works on permutation-based variable importance measures (VIMs) used in RF have come to apparently contradictory conclusions. We present an extended simulation study to synthesize results.},
    issn={1471-2105},
    doi={10.1186/1471-2105-11-110}
}

@article{Touw2013jungle,
  title={Data mining in the Life Sciences with Random Forest: a walk in the park or lost in the jungle?},
  author={W. G. Touw and others},
  journal={Briefings Bioinf.},
  year={2013},
  volume={14},
  pages={315 - 326}
}

@Article{Shi2005tumor,
    author={Shi, T.
    and Seligson, D.
    and Belldegrun, A. S.
    and Palotie, A.
    and Horvath, S.},
    title={Tumor classification by tissue microarray profiling: random forest clustering applied to renal cell carcinoma},
    journal={Mod. Pathol.},
    year={2005},
    month={Apr},
    day={01},
    volume={18},
    number={4},
    pages={547-557},
    abstract={We describe a novel strategy (random forest clustering) for tumor profiling based on tissue microarray data. Random forest clustering is attractive for tissue microarray and other immunohistochemistry data since it handles highly skewed tumor marker expressions well and weighs the contribution of each marker according to its relatedness with other tumor markers. This is the first tumor class discovery analysis of renal cell carcinoma patients based on protein expression profiles. The tissue array data contained at least three tumor samples from each of 366 renal cell carcinoma patients. The eight tumor markers explore tumor proliferation, cell cycle abnormalities, cell mobility, and the hypoxia pathway. Since the procedure is unsupervised, no clinicopathological data or traditional classifications are used a priori. To explore whether the tissue microarray data can be used to identify fundamental subtypes of renal cell carcinoma patients, we first carried out random forest clustering of all 366 patients. By analyzing the tumor markers simultaneously, the procedure automatically detected classes that correspond to clear- vs non-clear cell tumors (demonstration of proof-of-principle). The resulting molecular grouping provides better prediction of survival (logrank P=0.000090) than this classical pathological grouping (logrank P=0.023). We then sought to extend the class discovery by searching for finer subclasses of clear cell patients. The procedure automatically discovered: (a) two classes corresponding to low- and high-grade patients (demonstration of proof-of-principle); (b) a subgroup of long-surviving clear cell patients with a distinct molecular profile and (c) two novel tumor subclasses in low-grade clear cell patients that could not be explained by any clinicopathological variables (demonstration of discovery).},
    issn={1530-0285},
    doi={10.1038/modpathol.3800322},
    url={https://doi.org/10.1038/modpathol.3800322}
}

@article{horvath2006unsupervised,
    author = {T. Shi and S. Horvath},
    title = {Unsupervised Learning With Random Forest Predictors},
    journal = {J. Comput. Graphical Stat.},
    volume = {15},
    number = {1},
    pages = {118-138},
    year  = {2006},
    publisher = {Taylor & Francis},
    doi = {10.1198/106186006X94072},
    
    eprint = { 
            https://doi.org/10.1198/106186006X94072
        
    },
    url = {https://doi.org/10.1198/106186006X94072}
}

@article{finehout2007cerebrospinal,
	title = {Cerebrospinal fluid proteomic biomarkers for {Alzheimer}'s disease},
	volume = {61},
	issn = {03645134, 15318249},
	doi = {10.1002/ana.21038},
	language = {en},
	number = {2},
	urldate = {2021-01-15},
	journal = {Ann. Neurol.},
	author = {Finehout, E. J. and Franck, Z. and Choe, L. H. and Relkin, N. and Lee, K. H.},
	month = feb,
	year = {2007},
	pages = {120--129},
    url = {https://doi.org/10.1002/ana.21038}
}

@article{pang2006pathways,
    author = {Pang, H. and Lin, A. and Holford, M. and Enerson, B. E. and others},
    title = "{Pathway analysis using random forests classification and regression}",
    journal = {Bioinformatics},
    volume = {22},
    number = {16},
    pages = {2028-2036},
    year = {2006},
    month = {06},
    abstract = "{Motivation: Although numerous methods have been developed to better capture biological information from microarray data, commonly used single gene-based methods neglect interactions among genes and leave room for other novel approaches. For example, most classification and regression methods for microarray data are based on the whole set of genes and have not made use of pathway information. Pathway-based analysis in microarray studies may lead to more informative and relevant knowledge for biological researchers.Results: In this paper, we describe a pathway-based classification and regression method using Random Forests to analyze gene expression data. The proposed methods allow researchers to rank important pathways from externally available databases, discover important genes, find pathway-based outlying cases and make full use of a continuous outcome variable in the regression setting. We also compared Random Forests with other machine learning methods using several datasets and found that Random Forests classification error rates were either the lowest or the second-lowest. By combining pathway information and novel statistical methods, this procedure represents a promising computational strategy in dissecting pathways and can provide biological insight into the study of microarray data.Availability: Source code written in R is available from Contact:hongyu.zhao@yale.eduSupplementary Information: Supplementary Data are available at }",
    issn = {1367-4803},
    doi = {10.1093/bioinformatics/btl344},
    eprint = {https://academic.oup.com/bioinformatics/article-pdf/22/16/2028/548216/btl344.pdf},
    url = {http://doi.org/10.1093/bioinformatics/btl344}
}


@incollection{Cutler2012randomforests,
author="Cutler, Adele
and Cutler, D. Richard
and Stevens, John R.",
editor="Zhang, Cha
and Ma, Yunqian",
title="Random Forests",
bookTitle="Ensemble Machine Learning: Methods and Applications",
year="2012",
publisher="Springer US",
address="Boston, MA",
pages="157--175",
abstract="Random Forests were introduced by Leo Breiman [6] who was inspired by earlier work by Amit and Geman [2]. Although not obvious from the description in [6], Random Forests are an extension of Breiman's bagging idea [5] and were developed as a competitor to boosting. Random Forests can be used for either a categorical response variable, referred to in [6] as ``classification,'' or a continuous response, referred to as ``regression.'' Similarly, the predictor variables can be either categorical or continuous.",
isbn="978-1-4419-9326-7",
doi="10.1007/978-1-4419-9326-7-5",
url="https://doi.org/10.1007/978-1-4419-9326-7-5"
}




@Manual{R2021,
    title = {R: A Language and Environment for Statistical Computing},
    author = {{R Core Team}},
    organization = {R Foundation for Statistical Computing},
    address = {Vienna, Austria},
    year = {2019}
}

@Article{randomForest2021,
    title = {Classification and Regression by random{F}orest},
    author = {A. Liaw and M. Wiener},
    journal = {R News},
    year = {2002},
    volume = {2},
    number = {3},
    pages = {18-22}
}



@article{ishwaran2007vimp,
    author = "Ishwaran, H.",
    doi = "10.1214/07-EJS039",
    fjournal = "Electronic Journal of Statistics",
    journal = "Electron. J. Stat.",
    pages = "519--537",
    publisher = "The Institute of Mathematical Statistics and the Bernoulli Society",
    title = "Variable importance in binary regression trees and forests",
    volume = "1",
    year = "2007"
}

@Article{Strobl2008conditionalVIMP,
    author={Strobl, C.
    and Boulesteix, A.
    and Kneib, T.
    and Augustin, T.
    and Zeileis, A.},
    title={Conditional variable importance for random forests},
    journal={BMC Bioinf.},
    year={2008},
    month={Jul},
    day={11},
    volume={9},
    number={1},
    pages={307},
    abstract={Random forests are becoming increasingly popular in many scientific fields because they can cope with "small n large p" problems, complex interactions and even highly correlated predictor variables. Their variable importance measures have recently been suggested as screening tools for, e.g., gene expression studies. However, these variable importance measures show a bias towards correlated predictor variables.},
    issn={1471-2105},
    doi={10.1186/1471-2105-9-307}
}

@Article{Nicodemus2010permImpBehaviour,
    author={Nicodemus, K. K.
    and Malley, J. D.
    and Strobl, C.
    and Ziegler, A.},
    title={The behaviour of random forest permutation-based variable importance measures under predictor correlation},
    journal={BMC Bioinf.},
    year={2010},
    month={Feb},
    day={27},
    volume={11},
    pages={110},
    abstract={Random forests (RF) have been increasingly used in applications such as genome-wide association and microarray studies where predictor correlation is frequently observed. Recent works on permutation-based variable importance measures (VIMs) used in RF have come to apparently contradictory conclusions. We present an extended simulation study to synthesize results.},
    issn={1471-2105},
    doi={10.1186/1471-2105-11-110}
}

@article{pouyan2016distancelearning,
  title={Metric learning using random forest for cytometry data},
  author={Maziyar Baran Pouyan and Javad Birjandtalab and Mehrdad Nourani},
  journal={2016 38th Annual International Conference of the IEEE Engineering in Medicine and Biology Society (EMBC)},
  year={2016},
  pages={2590-2590},
  url = {http://doi.org/10.1109/EMBC.2016.7591260}
}
  
@ARTICLE{zhang2008Network,
  author={J. {Zhang} and M. {Zulkernine} and A. {Haque}},
  journal={IEEE Trans. Syst. Man Cybern., Part C (Applications and Reviews)}, 
  title={Random-Forests-Based Network Intrusion Detection Systems}, 
  year={2008},
  volume={38},
  number={5},
  pages={649-659},
  doi={10.1109/TSMCC.2008.923876}}

  
@incollection{hastie2017elements,
author="Hastie, Trevor
and Tibshirani, Robert
and Friedman, Jerome",
title="Random Forests",
bookTitle="The Elements of Statistical Learning: Data Mining, Inference, and Prediction",
year="2009",
publisher="Springer New York",
address="New York, NY",
pages="587--604",
isbn="978-0-387-84858-7",
doi="10.1007/978-0-387-84858-7-15",
url="https://doi.org/10.1007/978-0-387-84858-7\-15",
edition={2}
}
  
@article{gislason2006landcover,
    title = "Random Forests for land cover classification",
    journal = "Pattern Recognit. Lett.",
    volume = "27",
    number = "4",
    pages = "294 - 300",
    year = "2006",
    note = "Pattern Recognition in Remote Sensing (PRRS 2004)",
    issn = "0167-8655",
    doi = "10.1016/j.patrec.2005.08.011",
    author = "P. O. Gislason and J. A. Benediktsson and J. R. Sveinsson",
    keywords = "Random Forests, Classification, Decision trees, Multisource remote sensing data",
    abstract = "Random Forests are considered for classification of multisource remote sensing and geographic data. Various ensemble classification methods have been proposed in recent years. These methods have been proven to improve classification accuracy considerably. The most widely used ensemble methods are boosting and bagging. Boosting is based on sample re-weighting but bagging uses bootstrapping. The Random Forest classifier uses bagging, or bootstrap aggregating, to form an ensemble of classification and regression tree (CART)-like classifiers. In addition, it searches only a random subset of the variables for a split at each CART node, in order to minimize the correlation between the classifiers in the ensemble. This method is not sensitive to noise or overtraining, as the resampling is not based on weighting. Furthermore, it is computationally much lighter than methods based on boosting and somewhat lighter than simple bagging. In the paper, the use of the Random Forest classifier for land cover classification is explored. We compare the accuracy of the Random Forest classifier to other better-known ensemble methods on multisource remote sensing and geographic data."
    }
    
@article{Kokla2019metabolomicsimputation,
    author={Kokla, M.
    and Virtanen, J.
    and Kolehmainen, M.
    and Paananen, J.
    and Hanhineva, K.},
    title={Random forest-based imputation outperforms other methods for imputing {LC}-{MS} metabolomics data: a comparative study},
    journal={BMC Bioinf.},
    year={2019},
    month={Oct},
    day={11},
    volume={20},
    number={1},
    pages={492},
    abstract={LC-MS technology makes it possible to measure the relative abundance of numerous molecular features of a sample in single analysis. However, especially non-targeted metabolite profiling approaches generate vast arrays of data that are prone to aberrations such as missing values. No matter the reason for the missing values in the data, coherent and complete data matrix is always a pre-requisite for accurate and reliable statistical analysis. Therefore, there is a need for proper imputation strategies that account for the missingness and reduce the bias in the statistical analysis.},
    issn={1471-2105},
    doi={10.1186/s12859-019-3110-0},
    url = {http://doi.org/10.1186/s12859-019-3110-0}
}

@article{Hong2020imputationaccuracy,
    author={Hong, S.
    and Lynn, H. S.},
    title={Accuracy of random-forest-based imputation of missing data in the presence of non-normality, non-linearity, and interaction},
    journal={BMC Med. Res. Method.},
    year={2020},
    month={Jul},
    day={25},
    volume={20},
    number={1},
    pages={199},
    abstract={Missing data are common in statistical analyses, and imputation methods based on random forests (RF) are becoming popular for handling missing data especially in biomedical research. Unlike standard imputation approaches, RF-based imputation methods do not assume normality or require specification of parametric models. However, it is still inconclusive how they perform for non-normally distributed data or when there are non-linear relationships or interactions.},
    issn={1471-2288},
    doi={10.1186/s12874-020-01080-1},
    url = {http://doi.org/10.1186/s12874-020-01080-1}
}

@article{englund2012novelaproach,
    author = {Englund, C. and Verikas, A.},
    title = {A Novel Approach to Estimate Proximity in a Random Forest: An Exploratory Study},
    year = {2012},
    issue_date = {December, 2012},
    publisher = {Pergamon Press, Inc.},
    address = {USA},
    volume = {39},
    number = {17},
    issn = {0957-4174},
    doi = {10.1016/j.eswa.2012.05.094},
    url = {http://doi.org/10.1016/j.eswa.2012.05.094},
    abstract = {A data proximity matrix is an important information source in random forests (RF) based data mining, including data clustering, visualization, outlier detection, substitution of missing values, and finding mislabeled data samples. A novel approach to estimate proximity is proposed in this work. The approach is based on measuring distance between two terminal nodes in a decision tree. To assess the consistency (quality) of data proximity estimate, we suggest using the proximity matrix as a kernel matrix in a support vector machine (SVM), under the assumption that a matrix of higher quality leads to higher classification accuracy. It is experimentally shown that the proposed approach improves the proximity estimate, especially when RF is made of a small number of trees. It is also demonstrated that, for some tasks, an SVM exploiting the suggested proximity matrix based kernel, outperforms an SVM based on a standard radial basis function kernel and the standard proximity matrix based kernel.},
    journal = {Expert Syst. Appl.},
    month = dec,
    pages = {13046–13050},
    numpages = {5},
    keywords = {Kernel matrix, Proximity matrix, Random forest, Data mining, Support vector machine}
}

@misc{davies2014randomforestkernel,
      title={The Random Forest Kernel and other kernels for big data from random partitions}, 
      author={A. Davies and Z. Ghahramani},
      year={2014},
      eprint={1402.4293},
      archivePrefix={arXiv},
      primaryClass={stat.ML},
      url = {https://arxiv.org/abs/1402.4293}
}

@article{cao2019multi-viewradiomics,
    title = "Random forest dissimilarity based multi-view learning for Radiomics application",
    journal = "Pattern Recognit.",
    volume = "88",
    pages = "185 - 197",
    year = "2019",
    issn = "0031-3203",
    doi = "https://doi.org/10.1016/j.patcog.2018.11.011",
    author = "H. Cao and S. Bernard and R. Sabourin and L. Heutte",
    keywords = "Radiomics, Dissimilarity space, Random forest, Machine learning, Feature selection, Multi-view learning, High dimension, Low sample size",
    abstract = "Radiomics is a medical imaging technique that aims at extracting a large amount of features from one or several modalities of medical images, in order to help diagnose and treat diseases like cancers. Many recent studies have shown that Radiomics features can offer a lot of useful information that physicians cannot extract from these images, and can be efficiently associated with other information like gene or protein data. However, most of the classification studies in Radiomics report the use of feature selection methods without identifying the underlying machine learning challenges. In this paper, we first show that the Radiomics classification problem should be viewed as a high dimensional, low sample size, multi-view learning problem. Then, we propose a dissimilarity-based method for merging the information from the different views, based on Random Forest classifiers. The proposed approach is compared to different state-of-the-art Radiomics and multi-view solutions, on different public multi-view datasets as well as on Radiomics datasets. In particular, our experiments show that the proposed approach works better than the state-of-the-art methods from the Radiomics, as well as from the multi-view learning literature.",
    url={https://doi.org/10.1016/j.patcog.2018.11.011}
}


@article{Cao2020novelRFMV,
  title={A Novel Random Forest Dissimilarity Measure for Multi-View Learning},
  author={Hongliu Cao and Simon Bernard and Robert Sabourin and Laurent Heutte},
  journal={2020 25th Int. Conf. Pattern Recognit. (ICPR)},
  year={2021},
  pages={1344-1351},
  url = {http://doi.org/DOI:10.1109/ICPR48806.2021.9412961}
}

@misc{UCI2019,
author = "Dua, D. and Graff, C.",
year = "2017",
title = "{UCI} Machine Learning Repository",
institution = "University of California, Irvine, School of Information and Computer Sciences",
url = {http://archive.ics.uci.edu/ml},
note={(Accessed on 03/02/2023)}
}

@article{benali2019solar,
title = {Solar radiation forecasting using artificial neural network and random forest methods: Application to normal beam, horizontal diffuse and global components},
journal = {Renewable Energy},
volume = {132},
pages = {871-884},
year = {2019},
issn = {0960-1481},
doi = {10.1016/j.renene.2018.08.044},
author = {L. Benali and G. Notton and A. Fouilloy and C. Voyant and R. Dizene},
keywords = {Solar irradiation forecasting, ANN, Random forest, Beam solar radiation, Diffuse solar radiation, Global solar radiation},
abstract = {Three methods, smart persistence, artificial neural network and random forest, are compared to forecast the three components of solar irradiation (global horizontal, beam normal and diffuse horizontal) measured on the site of Odeillo, France, characterized by a high meteorological variability. The objective is to predict hourly solar irradiations for time horizons from h+1 to h+6. The random forest (RF) method is the most efficient and forecasts the three components with a nRMSE from 19.65\% for h+1–27.78\% for h+6 for the global horizontal irradiation (GHI), a nRMSE from 34.11\% for h+1–49.08\% for h+6 for the beam normal irradiation (BNI); a nRMSE from 35.08\% for h+1–49.14\% for h+6 for diffuse horizontal irradiation (DHI). The improvement brought by the use of RF compared to Artificial Neural Network (ANN) and smart persistence (SP) increases with the forecasting horizon. A seasonal study is realized and shows that the forecasting of solar irradiation during spring and autumn is less reliable than during winter and summer because during these periods the meteorological variability is more important.},
url={https://doi.org/10.1016/j.renene.2018.08.044}
}

@article{Han2018ComparisonOR,
  title={Comparison of random forest, artificial neural networks and support vector machine for intelligent diagnosis of rotating machinery},
  author={T. Han and D. Jiang and Q. Zhao and L. Wang and Kai Yin},
  journal={Trans. Inst. Meas. Control},
  year={2018},
  volume={40},
  pages={2681 - 2693},
  url={https://doi.org/10.1177/0142331217708242}
}

@ARTICLE{iwendi2020covid,
AUTHOR={Iwendi, Celestine and Bashir, Ali Kashif and Peshkar, Atharva and Sujatha, R. and Chatterjee, Jyotir Moy and Pasupuleti, Swetha and Mishra, Rishita and Pillai, Sofia and Jo, Ohyun},   
TITLE={{COVID}-19 Patient Health Prediction Using Boosted Random Forest Algorithm},      
JOURNAL={Front. Public Health},      
VOLUME={8},      
PAGES={357},     
YEAR={2020},      
DOI={10.3389/fpubh.2020.00357},      
ISSN={2296-2565},   
ABSTRACT={Integration of artificial intelligence (AI) techniques in wireless infrastructure, real-time collection, and processing of end-user devices is now in high demand. It is now superlative to use AI to detect and predict pandemics of a colossal nature. The Coronavirus disease 2019 (COVID-19) pandemic, which originated in Wuhan China, has had disastrous effects on the global community and has overburdened advanced healthcare systems throughout the world. Globally; over 4,063,525 confirmed cases and 282,244 deaths have been recorded as of 11th May 2020, according to the European Centre for Disease Prevention and Control agency. However, the current rapid and exponential rise in the number of patients has necessitated efficient and quick prediction of the possible outcome of an infected patient for appropriate treatment using AI techniques. This paper proposes a fine-tuned Random Forest model boosted by the AdaBoost algorithm. The model uses the COVID-19 patient's geographical, travel, health, and demographic data to predict the severity of the case and the possible outcome, recovery, or death. The model has an accuracy of 94\% and a F1 Score of 0.86 on the dataset used. The data analysis reveals a positive correlation between patients' gender and deaths, and also indicates that the majority of patients are aged between 20 and 70 years.},
url={https://doi.org/10.3389/fpubh.2020.00357}
}

@article{YESILKANAT2020covidSpac,
title = {Spatio-temporal estimation of the daily cases of {COVID}-19 in worldwide using random forest machine learning algorithm},
journal = {Chaos, Solitons Fractals},
volume = {140},
pages = {110210},
year = {2020},
issn = {0960-0779},
doi = {10.1016/j.chaos.2020.110210},
url = {https://doi.org/10.1016/j.chaos.2020.110210},
author = {C. M. Yeşilkanat},
keywords = {COVID-19, Random forest, Machine learning, Estimating, Mapping},
abstract = {Novel Coronavirus pandemic, which negatively affected public health in social, psychological and economical terms, spread to the whole world in a short period of 6 months. However, the rate of increase in cases was not equal for every country. The measures implemented by the countries changed the daily spreading speed of the disease. This was determined by changes in the number of daily cases. In this study, the performance of the Random Forest (RF) machine learning algorithm was investigated in estimating the near future case numbers for 190 countries in the world and it is mapped in comparison with actual confirmed cases results. The number of confirmed cases between 23/01/2020 - 17/06/2020 were divided into 3 main sub-datasets: training sub-data, testing sub-data (interpolation data) and estimating sub-data (extrapolation data) for the random forest model. At the end of the study, it has been found that R2 values for testing sub-data of RF model estimates range between 0.843 and 0.995 (average R2= 0.959), and RMSE values between 141.76 and 526.18 (mean RMSE = 259.38); and that R2 values for estimating sub-data range between 0.690 and 0.968 (mean R2 = 0.914), and RMSE values between 549.73 and 2500.79 (mean RMSE = 909.37). These results show that the random forest machine learning algorithm performs well in estimating the number of cases for the near future in case of an epidemic like Novel Coronavirus, which outbreaks suddenly and spreads rapidly.}
}


@Article{nhu2020landslide,
AUTHOR = {Nhu, V. and Shirzadi, A. and Shahabi, H. and Chen, W. and Clague, J. J. and Geertsema and others},
TITLE = {Shallow Landslide Susceptibility Mapping by Random Forest Base Classifier and Its Ensembles in a Semi-Arid Region of {I}ran},
JOURNAL = {Forests},
VOLUME = {11},
YEAR = {2020},
NUMBER = {4},
ARTICLE-NUMBER = {421},
ISSN = {1999-4907},
ABSTRACT = {We generated high-quality shallow landslide susceptibility maps for Bijar County, Kurdistan Province, Iran, using Random Forest (RAF), an ensemble computational intelligence method and three meta classifiers&mdash;Bagging (BA, BA-RAF), Random Subspace (RS, RS-RAF), and Rotation Forest (RF, RF-RAF). Modeling and validation were done on 111 shallow landslide locations using 20 conditioning factors tested by the Information Gain Ratio (IGR) technique. We assessed model performance with statistically based indexes, including sensitivity, specificity, accuracy, kappa, root mean square error (RMSE), and area under the receiver operatic characteristic curve (AUC). All four machine learning models that we tested yielded excellent goodness-of-fit and prediction accuracy, but the RF-RAF ensemble model (AUC = 0.936) outperformed the BA-RAF, RS-RAF (AUC = 0.907), and RAF (AUC = 0.812) models. The results also show that the Random Forest model significantly improved the predictive capability of the RAF-based classifier and, therefore, can be considered as a useful and an effective tool in regional shallow landslide susceptibility mapping.},
DOI = {10.3390/f11040421},
url = {https://doi.org/10.3390/f11040421}
}

@Article{Fang2020diar,
author={Fang, X.
and Liu, We.
and Ai, J.
and He, M.
and Wu, Y.},
title={Forecasting incidence of infectious diarrhea using random forest in {J}iangsu Province, {C}hina},
journal={BMC Infect. Dis.},
year={2020},
month={Mar},
day={14},
volume={20},
number={1},
pages={222},
abstract={Infectious diarrhea can lead to a considerable global disease burden. Thus, the accurate prediction of an infectious diarrhea epidemic is crucial for public health authorities. This study was aimed at developing an optimal random forest (RF) model, considering meteorological factors used to predict an incidence of infectious diarrhea in Jiangsu Province, China.},
issn={1471-2334},
doi={10.1186/s12879-020-4930-2},
url = {https://doi.org/10.1186/s12879-020-4930-2}
}

@Article{Yang2020cardio,
author={Yang, L.
and Wu, H.
and Jin, X.
and Zheng, P.
and Hu, S.
and Xu, X.
and Yu, W.
and Yan, J.},
title={Study of cardiovascular disease prediction model based on random forest in eastern {C}hina},
journal={Sci. Rep.},
year={2020},
month={Mar},
day={23},
volume={10},
number={1},
pages={5245},
abstract={Cardiovascular disease (CVD) is the leading cause of death worldwide and a major public health concern. CVD prediction is one of the most effective measures for CVD control. In this study, 29930 subjects with high-risk of CVD were selected from 101056 people in 2014, regular follow-up was conducted using electronic health record system. Logistic regression analysis showed that nearly 30 indicators were related to CVD, including male, old age, family income, smoking, drinking, obesity, excessive waist circumference, abnormal cholesterol, abnormal low-density lipoprotein, abnormal fasting blood glucose and else. Several methods were used to build prediction model including multivariate regression model, classification and regression tree (CART), Na{\"i}ve Bayes, Bagged trees, Ada Boost and Random Forest. We used the multivariate regression model as a benchmark for performance evaluation (Area under the curve, AUC{\thinspace}={\thinspace}0.7143). The results showed that the Random Forest was superior to other methods with an AUC of 0.787 and achieved a significant improvement over the benchmark. We provided a CVD prediction model for 3-year risk assessment of CVD. It was based on a large population with high risk of CVD in eastern China using Random Forest algorithm, which would provide reference for the work of CVD prediction and treatment in China.},
issn={2045-2322},
doi={10.1038/s41598-020-62133-5},
url={https://doi.org/10.1038/s41598-020-62133-5}
}


@article{saha2020deforest,
title = {Predicting the deforestation probability using the binary logistic regression, random forest, ensemble rotational forest, {REPT}ree: A case study at the {G}umani {R}iver {B}asin, {I}ndia},
journal = {Sci. Total Environ.},
volume = {730},
pages = {139197},
year = {2020},
issn = {0048-9697},
doi = {10.1016/j.scitotenv.2020.139197},
url = {https://doi.org/10.1016/j.scitotenv.2020.139197},
author = {S. Saha and M. Saha and K. Mukherjee and A. Arabameri and P. T. T. Ngo and G. C. Paul},
keywords = {Forest canopy density, Deforestation, Machine learning algorithms, Probabilistic model, Ensemble model},
abstract = {Rapid population growth and its corresponding effects like the expansion of human settlement, increasing agricultural land, and industry lead to the loss of forest area in most parts of the world especially in such highly populated nations like India. Forest canopy density (FCD) is a useful measure to assess the forest cover change in its own as numerous works of forest change have been done using only FCD with the help of remote sensing and GIS. The coupling of binary logistic regression (BLR), random forest (RF), ensemble of rotational forest and reduced error pruning trees (RTF-REPTree) with FCD makes it more convenient to find out the deforestation probability. Advanced vegetation index (AVI), bare soil index (BSI), shadow index (SI), and scaled vegetation density (VD) derived from Landsat imageries are the main input parameters to identify the FCD. After preparing the FCDs of 1990, 2000, 2010 and 2017 the deforestation map of the study area was prepared and considered as dependent parameter for deforestation probability modelling. On the other hand, twelve deforestation determining factors were used to delineate the deforestation probability with the help of BLR, RF and RTF-REPTree models. These deforestation probability models were validated through area under curve (AUC), receiver operating characteristics (ROC), efficiency, true skill statistics (TSS) and Kappa co-efficient. The validation result shows that all the models like BLR (AUC = 0.874), RF (AUC = 0.886) and RTF-REPTree (AUC = 0.919) have good capability of assessing the deforestation probability but among them, RTF-REPTree has the highest accuracy level. The result also shows that low canopy density area i.e. not under the dense forest cover has increased by 9.26\% from 1990 to 2017. Besides, nearly 30\% of the forested land is under high to very high deforestation probable zone, which needs to be protected with immediate measures.}
}

@article{GHOLIZADEH2020nanofluid,
title = {Prediction of nanofluids viscosity using random forest ({RF}) approach},
journal = {Chemom. Intell. Lab. Syst.},
volume = {201},
pages = {104010},
year = {2020},
issn = {0169-7439},
doi = {10.1016/j.chemolab.2020.104010},
url = {https://doi.org/10.1016/j.chemolab.2020.104010},
author = {M. Gholizadeh and M. Jamei and I. Ahmadianfar and R. Pourrajab},
keywords = {Relative viscosity, Nanofluid, Nanoparticle, RF, SVR, MLP}
}

@article{rao2020credit,
title = {2-stage modified random forest model for credit risk assessment of P2P network lending to “Three Rurals” borrowers},
journal = {Appl. Soft Comput.},
volume = {95},
pages = {106570},
year = {2020},
issn = {1568-4946},
doi = {10.1016/j.asoc.2020.106570},
url = {https://doi.org/10.1016/j.asoc.2020.106570},
author = {C. Rao and M. Liu and M. Goh and J. Wen},
keywords = {P2P network lending, ”Three Rurals” borrowers, Credit risk evaluation, Random forest},
abstract = {With the rapid growth of the P2P online loan industry in the “Three Rurals” (agriculture, rural areas, and farmers) sector, it is imperative to manage the borrowing risk of borrowers in the rural areas. A credit risk assessment model is proposed to classify the credit worthiness of the “Three Rurals” borrowers. We select the loan data of the Pterosaur Loan platform as the research sample, and establish a 2-stage Syncretic Cost-sensitive Random Forest (SCSRF) model to evaluate the credit risk of the borrowers. From the random forest, we construct a cost relationship from the actual distribution of the data categories, introduce a weighted Mahalanobis distance using the entropy weight method in the cost function, and adopt a weighted voting for the cost-sensitive decision tree base classifier. The parameters of the SCSRF model are optimized via a grid search. We validate the SCSRF classification model against several established credit evaluation models.}
}

@Article{Lv2020rna,
author={Lv, Z.
and Zhang, J.
and Ding, H.
and Zou, Q.},
title={{RF}-{P}se{U}: A Random Forest Predictor for RNA Pseudouridine Sites},
journal={Front. Bioeng. Biotechnol.},
year={2020},
month={Feb},
day={26},
publisher={Frontiers Media S.A.},
volume={8},
pages={134-134},
keywords={RNA; light gradient boosting; machine learning; pseudouridine sites; random forest},
abstract={One of the ubiquitous chemical modifications in RNA, pseudouridine modification is crucial for various cellular biological and physiological processes. To gain more insight into the functional mechanisms involved, it is of fundamental importance to precisely identify pseudouridine sites in RNA. Several useful machine learning approaches have become available recently, with the increasing progress of next-generation sequencing technology; however, existing methods cannot predict sites with high accuracy. Thus, a more accurate predictor is required. In this study, a random forest-based predictor named RF-PseU is proposed for prediction of pseudouridylation sites. To optimize feature representation and obtain a better model, the light gradient boosting machine algorithm and incremental feature selection strategy were used to select the optimum feature space vector for training the random forest model RF-PseU. Compared with previous state-of-the-art predictors, the results on the same benchmark data sets of three species demonstrate that RF-PseU performs better overall. The integrated average leave-one-out cross-validation and independent testing accuracy scores were 71.4{\%} and 74.7{\%}, respectively, representing increments of 3.63{\%} and 4.77{\%} versus the best existing predictor. Moreover, the final RF-PseU model for prediction was built on leave-one-out cross-validation and provides a reliable and robust tool for identifying pseudouridine sites. A web server with a user-friendly interface is accessible at http://148.70.81.170:10228/rfpseu.},
issn={2296-4185},
doi={10.3389/fbioe.2020.00134},
language={eng},
url={https://doi.org/10.3389/fbioe.2020.00134}
}

@article{tahir2020sensor,
  title={Wearable Sensors for Activity Analysis using {SMO}-based Random Forest over Smart home and Sports Datasets},
  author={Sheikh Badar ud din Tahir and Ahmad Jalal and Mouazma Batool},
  journal={2020 3rd International Conference on Advancements in Computational Sciences (ICACS)},
  year={2020},
  pages={1-6},
  url={http://doi.org/10.1109/ICACS47775.2020.9055944}
}


@article{tan2020soil,
title = {Estimation of the spatial distribution of heavy metal in agricultural soils using airborne hyperspectral imaging and random forest},
journal = {J. Hazard. Mater.},
volume = {382},
pages = {120987},
year = {2020},
issn = {0304-3894},
doi = {10.1016/j.jhazmat.2019.120987},
url = {https://doi.org/10.1016/j.jhazmat.2019.120987},
author = {K. Tan and H. Wang and L. Chen and Q. Du and P. Du and C. Pan},
keywords = {Airborne hyperspectral remote sensing, Random forest, Soil heavy metal},
abstract = {Hyperspectral imaging, with the hundreds of bands and high spectral resolution, offers a promising approach for estimation of heavy metal concentration in agricultural soils. Using airborne imagery over a large-scale area for fast retrieval is of great importance for environmental monitoring and further decision support. However, few studies have focused on the estimation of soil heavy metal concentration by airborne hyperspectral imaging. In this study, we utilized the airborne hyperspectral data in LiuXin Mine of China obtained from HySpex VNIR-1600 and HySpex SWIR-384 sensor to establish the spectral-analysis-based model for retrieval of heavy metals concentration. Firstly, sixty soil samples were collected in situ, and their heavy metal concentrations (Cr, Cu, Pb) were determined by inductively coupled plasma-mass spectrometry analysis. Due to mixed pixels widespread in airborne hyperspectral images, spectral unmixing was conducted to obtain purer spectra of the soil and to improve the estimation accuracy. Ten of estimated models, including four different random forest models (RF)—standard random forest (SRF), regularized random forest (RRF), guided random forest (GRF), and guided regularized random forest (GRRF)—were introduced for hyperspectral estimated model in this paper. Compared with the estimation results, the best accuracy for Cr, Cu, and Pb is obtained by RF. It shows that RF can predict the three heavy metals better than other models in this area. For Cr, Cu, Pb, the best model of RF yields Rp2 values of 0.75,0.68 and 0.74 respectively, and the values of RMSEp are 5.62, 8.24, and 2.81 (mg/kg), respectively. The experiments show the average estimated values are close to the truth condition and the high estimated values concentrated near several industries, valifating the effectiveness of the presented method.}
}

@article{nesa2018iot,
  title={Outlier detection in sensed data using statistical learning models for {I}o{T}},
  author={Nashreen Nesa and Tania Ghosh and Indrajit Banerjee},
  journal={2018 IEEE Wireless Communications and Networking Conference (WCNC)},
  year={2018},
  pages={1-6},
  doi={10.1109/WCNC.2018.8376988},
  url = {http://doi.org/10.1109/WCNC.2018.8376988}
}
  
@article{liu2018species,
    author = {Liu, C. and White, M. and Newell, G.},
    title = {Detecting outliers in species distribution data},
    journal = {J. Biogeogr.},
    volume = {45},
    number = {1},
    pages = {164-176},
    keywords = {outlier, outlier detection, random forest, species distribution, species distribution modelling, support vector machine, virtual species},
    url = {https://doi.org/10.1111/jbi.13122},
    doi = {10.1111/jbi.13122},
    eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1111/jbi.13122},
    year = {2018}
}

@article{santana2019foodadult,
title = {Random forest as one-class classifier and infrared spectroscopy for food adulteration detection},
journal = {Food Chem.},
volume = {293},
pages = {323-332},
year = {2019},
issn = {0308-8146},
doi = {10.1016/j.foodchem.2019.04.073},
url = {https://doi.org/10.1016/j.foodchem.2019.04.073},
author = {F. B. {de Santana} and W. {Borges Neto} and R. J. Poppi},
keywords = {One-class, Random forest, Artificial outliers, Food adulteration, Infrared spectroscopy},
abstract = {This paper proposes the use of random forest for adulteration detection purposes, combining the random forest algorithm with the artificial generation of outliers from the authentic samples. This proposal was applied in two food adulteration studies: evening primrose oils using ATR-FTIR spectroscopy and ground nutmeg using NIR diffuse reflectance spectroscopy. The primrose oil was adulterated with soybean, corn and sunflower oils, and the model was validated using these adulterated oils and other different oils, such as rosehip and andiroba, in pure and adulterated forms. The ground nutmeg was adulterated with cumin, commercial monosodium glutamate, soil, roasted coffee husks and wood sawdust. For the primrose oil, the proposed method presented superior performance than PLS-DA and similar performance to SIMCA and for the ground nutmeg, the random forest was superior to PLS-DA and SIMCA. Also, in both applications using the random forest, no sample was excluded from the external validation set.}
}

@article{baron2016galaxy,
    author = {Baron, D. and Poznanski, D.},
    title = "{The weirdest SDSS galaxies: results from an outlier detection algorithm}",
    journal = {Mon. Not. R. Astron. Soc.},
    volume = {465},
    number = {4},
    pages = {4530-4555},
    year = {2016},
    month = {11},
    abstract = "{How can we discover objects we did not know existed within the large data sets that now abound in astronomy? We present an outlier detection algorithm that we developed, based on an unsupervised Random Forest. We test the algorithm on more than two million galaxy spectra from the Sloan Digital Sky Survey and examine the 400 galaxies with the highest outlier score. We find objects which have extreme emission line ratios and abnormally strong absorption lines, objects with unusual continua, including extremely reddened galaxies. We find galaxy–galaxy gravitational lenses, double-peaked emission line galaxies and close galaxy pairs. We find galaxies with high ionization lines, galaxies that host supernovae and galaxies with unusual gas kinematics. Only a fraction of the outliers we find were reported by previous studies that used specific and tailored algorithms to find a single class of unusual objects. Our algorithm is general and detects all of these classes, and many more, regardless of what makes them peculiar. It can be executed on imaging, time series and other spectroscopic data, operates well with thousands of features, is not sensitive to missing values and is easily parallelizable.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/stw3021},
    url = {http://doi.org/10.1093/mnras/stw3021},
    eprint = {https://academic.oup.com/mnras/article-pdf/465/4/4530/10254645/stw3021.pdf},
}

@article{vejendla2020network,
title = {Accurate identification and detection of outliers in networks using group random forest methodoly},
journal = {J. Crit. Rev.},
year = {2020},
volume = {7},
number = {6},
pages = {381-384},
author = {Narayana, V.L. and Gopi, A.P. and Khadherbhi, S.R. and Pavani, V.},
url = {http://doi.org/10.31838/jcr.07.06.67}
}

@InProceedings{pantanowitz2009missingdata,
    author="Pantanowitz, A.
    and Marwala, T.",
    editor="Yu, W.
    and Sanchez, E. N.",
    title="Missing Data Imputation Through the Use of the Random Forest Algorithm",
    booktitle= "Advances in Computational Intelligence",
    year="2009",
    publisher="Springer",
    address="Berlin, Heidelberg",
    pages="53--62",
    abstract="This paper presents a comparison of different paradigms used for missing data imputation. The data set used is HIV seroprevalence data from an antenatal clinic study survey performed in 2001. Data imputation is performed through five methods: Random Forests; auto-associative neural networks with genetic algorithms; auto-associative neuro-fuzzy configurations; and two random forest and neural network based hybrids. Results indicate that Random Forests are superior in imputing missing data for the given data set in terms of accuracy and in terms of computation time, with accuracy increases of up to 32 {\%} on average for certain variables when compared with auto-associative networks. While the concept of hybrid systems has promise, the presented systems appear to be hindered by their auto-associative neural network components.",
    isbn="978-3-642-03156-4",
    url = {http://doi.org/10.1007/978-3-642-03156-4-6}
}

@Article{Shah2014caliber,
author={Shah, A. D.
and Bartlett, J. W.
and Carpenter, J.
and Nicholas, O.
and Hemingway, H.},
title={Comparison of random forest and parametric imputation models for imputing missing data using {MICE}: a CALIBER study},
journal={Am. J. Epidemiol.},
year={2014},
month={Mar},
day={15},
edition={2014/01/12},
publisher={Oxford University Press},
volume={179},
number={6},
pages={764-774},
keywords={angina, stable; imputation; missing data; missingness at random; regression trees; simulation; survival; Age Factors; Angina, Stable/epidemiology; *Artificial Intelligence; Bias; *Computer Simulation; Confidence Intervals; *Epidemiologic Methods; Health Behavior; Health Status; Humans; Proportional Hazards Models; Random Allocation; Sex Factors},
abstract={Multivariate imputation by chained equations (MICE) is commonly used for imputing missing data in epidemiologic research. The "true" imputation model may contain nonlinearities which are not included in default imputation models. Random forest imputation is a machine learning technique which can accommodate nonlinearities and interactions and does not require a particular regression model to be specified. We compared parametric MICE with a random forest-based MICE algorithm in 2 simulation studies. The first study used 1,000 random samples of 2,000 persons drawn from the 10,128 stable angina patients in the CALIBER database (Cardiovascular Disease Research using Linked Bespoke Studies and Electronic Records; 2001-2010) with complete data on all covariates. Variables were artificially made "missing at random," and the bias and efficiency of parameter estimates obtained using different imputation methods were compared. Both MICE methods produced unbiased estimates of (log) hazard ratios, but random forest was more efficient and produced narrower confidence intervals. The second study used simulated data in which the partially observed variable depended on the fully observed variables in a nonlinear way. Parameter estimates were less biased using random forest MICE, and confidence interval coverage was better. This suggests that random forest imputation may be useful for imputing complex epidemiologic data sets in which some patients have missing data.},
issn={1476-6256},
doi={10.1093/aje/kwt312},
language={eng},
url = {http://doi.org/10.1093/aje/kwt312}
}

@Article{Ramosaj2019predictmiss,
author={Ramosaj, B.
and Pauly, M.},
title={Predicting missing values: a comparative study on non-parametric approaches for imputation},
journal={Comput. Stat.},
year={2019},
month={Dec},
day={01},
volume={34},
number={4},
pages={1741-1764},
abstract={Missing data is an expected issue when large amounts of data is collected, and several imputation techniques have been proposed to tackle this problem. Beneath classical approaches such as MICE, the application of Machine Learning techniques is tempting. Here, the recently proposed missForest imputation method has shown high imputation accuracy under the Missing (Completely) at Random scheme with various missing rates. In its core, it is based on a random forest for classification and regression, respectively. In this paper we study whether this approach can even be enhanced by other methods such as the stochastic gradient tree boosting method, the C5.0 algorithm, BART or modified random forest procedures. In particular, other resampling strategies within the random forest protocol are suggested. In an extensive simulation study, we analyze their performances for continuous, categorical as well as mixed-type data. An empirical analysis focusing on credit information and Facebook data complements our investigations.},
issn={1613-9658},
doi={10.1007/s00180-019-00900-3}
}

@article{narayana2020outlierdet,
  title={Accurate identification and detection of outliers in networks using group random forest methodoly},
  author={Narayana, V. L. and Gopi, A. P. and Khadherbhi, S. R. and Pavani, V},
  journal={J. Crit. Rev.},
  volume={7},
  number={6},
  pages={381--384},
  year={2020},
  publisher={Innovare Academics Sciences}
}


@Article{Moon2019phate,
    author={Moon, K. R.
    and van Dijk, D.
    and Wang, Z.
    and Gigante, S.
    and Burkhardt, D. B.
    and Chen, W. S.
    and Yim, K.
    and Elzen, A.
    and Hirn, M. J.
    and Coifman, R. R.
    and Ivanova, N. B.
    and Wolf, G.
    and Krishnaswamy, S.},
    title={Visualizing structure and transitions in high-dimensional biological data},
    journal={Nat. Biotechnol.},
    year={2019},
    month={Dec},
    day={01},
    volume={37},
    number={12},
    pages={1482-1492},
    url={https://doi.org/10.1038/s41587-019-0336-3}
}


@article{vanDerMaaten2008tsne,
  author = {van der Maaten, L. and Hinton, G.},
  journal = {J. Mach. Learn. Res.},
  keywords = {dimensionality reduction tSNE visualization},
  pages = {2579--2605},
  timestamp = {2015-08-19T15:19:11.000+0200},
  title = {Visualizing Data using {t-SNE} },
  volume = 9,
  year = 2008,
  url  = {http://jmlr.org/papers/v9/vandermaaten08a.html}
}



@book{KruskalWish1978mds,
  title={Multidimensional Scaling},
  author={Kruskal, J.B. and Wish, M.},
  number={11},
  isbn={9780803909403},
  lccn={77093286},
  series={Multidimensional Scaling},
  year={1978},
  publisher={Sage Publications},
  address={Newbury Park, California}
}




@article{lel2018umap,
    title={{UMAP: U}niform Manifold Approximation and Projection for Dimension Reduction},
    author={L. McInnes and J. Healy and J. Melville},
    year={2018},
    volume={abs/1802.03426},
    journal={arXiv},
    url = {https://arxiv.org/abs/1802.03426}
}

@article{duque2020grae,
  title={Extendable and invertible manifold learning with geometry regularized autoencoders},
  author={Andr'es F. Duque and Sacha Morin and Guy Wolf and Kevin R. Moon},
  journal={2020 IEEE International Conference on Big Data (Big Data)},
  year={2020},
  pages={5027-5036},
  url = {http://doi.org/10.1109/BigData50022.2020.9378049}
}
  
 @article {Tenenbaum2000isomap,
	author = {Tenenbaum, J. B. and Silva, V. and Langford, J. C.},
	title = {A Global Geometric Framework for Nonlinear Dimensionality Reduction},
	volume = {290},
	number = {5500},
	pages = {2319--2323},
	year = {2000},
	doi = {},
	journal = {Science},
    url = {https://doi.org/10.1126/science.290.5500.2319}
}


@Article{Cortes1995svm,
author={Cortes, C.
and Vapnik, V.},
title={Support-vector networks},
journal={Mach. Learn.},
year={1995},
month={Sep},
day={01},
volume={20},
number={3},
pages={273-297},
abstract={The support-vector network is a new learning machine for two-group classification problems. The machine conceptually implements the following idea: input vectors are non-linearly mapped to a very high-dimension feature space. In this feature space a linear decision surface is constructed. Special properties of the decision surface ensures high generalization ability of the learning machine. The idea behind the support-vector network was previously implemented for the restricted case where the training data can be separated without errors. We here extend this result to non-separable training data.},
issn={1573-0565},
doi={10.1007/BF00994018}
}


@book{Scholkopf99kernelprincipal,
editor = {Sch\"{o}lkopf, Bernhard and Burges, Christopher J. C. and Smola, Alexander J.},
title = {Advances in Kernel Methods: Support Vector Learning},
year = {1999},
isbn = {0262194163},
publisher = {MIT Press},
address = {Cambridge, MA, USA}
}

@article{ng2001spectral,
  title={On spectral clustering: Analysis and an algorithm},
  author={Ng, A. and Jordan, M. and Weiss, Y.},
  journal={Adv. Neural. Inf. Process. Syst.},
  volume={14},
  pages={849--856},
  year={2001}
}


@Article{rhodes2021rfphate,
author={Rhodes, Jake S.
and Cutler, Adele
and Wolf, Guy
and Moon, Kevin R.},
title={Random Forest-Based Diffusion Information Geometry for Supervised Visualization and Data Exploration},
journal={2021 IEEE Statistical Signal Processing Workshop (SSP)},
year={2021},
publisher={IEEE},
pages={331-335},
keywords={data reduction; data visualisation; image classification; learning (artificial intelligence); pattern classification; principal component analysis; class labels; increased classification accuracy; improved data visualization; visualization technique; random forest proximities; diffusion-based information geometry; supervised task; reliable visualizations; data exploration; random forest-based diffusion information geometry; supervised visualization; dimensionality reduction techniques; important patterns; supervised dimensionality reduction methods; account auxiliary annotations; Dimensionality reduction; Information geometry; Data visualization; Signal processing algorithms; Signal processing; Reliability; Task analysis},
abstract={Most dimensionality reduction techniques to date are unsupervised; they do not take class labels into account (e.g., PCA, MDS, t-SNE, Isomap). Such methods require large amounts of data and are often sensitive to noise that may obfuscate important patterns in the data. Various attempts at supervised dimensionality reduction methods that take into account auxiliary annotations (e.g., class labels) have been successfully implemented with goals of increased classification accuracy or improved data visualization. In this paper, we describe a novel supervised visualization technique based on random forest proximities and a diffusion-based information geometry. We show, both qualitatively and quantitatively, the advantages of our approach in retaining local and global structure in data, while demonstrating the spatial relevance of features important for the supervised task. Importantly, our approach is robust to noise and parameter tuning, thus making it simple to use while producing reliable visualizations for data exploration.},
doi={10.1109/SSP49050.2021.9513749},
url={https://doi.org/10.1109/SSP49050.2021.9513749}
}


@article{vanburren2011mice,
   author = {S. van Buuren and K. Groothuis-Oudshoorn},
   title = {mice: Multivariate Imputation by Chained Equations in {R}},
   journal = {J. Stat. Softw.},
   volume = {45},
   number = {3},
   year = {2011},
   keywords = {},
   abstract = {The R package mice imputes incomplete multivariate data by chained equations. The software mice 1.0 appeared in the year 2000 as an S-PLUS library, and in 2001 as an R package. mice 1.0 introduced predictor selection, passive imputation and automatic pooling. This article documents mice, which extends the functionality of mice 1.0 in several ways. In mice, the analysis of imputed data is made completely general, whereas the range of models under which pooling works is substantially extended. mice adds new functionality for imputing multilevel data, automatic predictor selection, data handling, post-processing imputed values, specialized pooling routines, model selection tools, and diagnostic graphs. Imputation of categorical data is improved in order to bypass problems caused by perfect prediction. Special attention is paid to transformations, sum scores, indices and interactions using passive imputation, and to the proper setup of the predictor matrix. mice can be downloaded from the Comprehensive R Archive Network. This article provides a hands-on, stepwise approach to solve applied incomplete data problems.},
   issn = {1548-7660},
   pages = {1--67},
   doi = {10.18637/jss.v045.i03},
   url = {http://doi.org/10.18637/jss.v045.i03}
}

  @Article{wright2017ranger,
    title = {{ranger}: A Fast Implementation of Random Forests for High
      Dimensional Data in {C++} and {R}},
    author = {M. N. Wright and A. Ziegler},
    journal = {J. Stat. Softw.},
    year = {2017},
    volume = {77},
    number = {1},
    pages = {1--17},
    doi = {10.18637/jss.v077.i01},
  }
  
  @article{deng2012mnist,
      title={The mnist database of handwritten digit images for machine learning research},
      author={Deng, Li},
      journal={IEEE Signal Process. Mag.},
      volume={29},
      number={6},
      pages={141--142},
      year={2012},
      publisher={IEEE}
}

@ARTICLE{hearst1998svm,
  author={Hearst, M.A. and Dumais, S.T. and Osuna, E. and Platt, J. and Scholkopf, B.},
  journal={IEEE Intell. Syst.}, 
  title={Support vector machines}, 
  year={1998},
  volume={13},
  number={4},
  pages={18-28},
  doi={10.1109/5254.708428},
  url={http://doi.org/10.1109/5254.708428}}
  
  

@inproceedings{arjovsky2017wasserstein,
author = {Arjovsky, Martin and Chintala, Soumith and Bottou, L\'{e}on},
title = {Wasserstein Generative Adversarial Networks},
year = {2017},
publisher = {JMLR.org},
abstract = {We introduce a new algorithm named WGAN, an alternative to traditional GAN training. In this new model, we show that we can improve the stability of learning, get rid of problems like mode collapse, and provide meaningful learning curves useful for debugging and hyperparameter searches. Furthermore, we show that the corresponding optimization problem is sound, and provide extensive theoretical work highlighting the deep connections to different distances between distributions.},
booktitle = {Proceedings of the 34th Int. Conf. on Mach. Learn. - Volume 70},
pages = {214–223},
numpages = {10},
location = {Sydney, NSW, Australia},
series = {ICML'17}
}



@InProceedings{Ribeiro2008esiso,
author="Ribeiro, Bernardete
and Vieira, Armando
and Carvalho das Neves, Jo{\~a}o",
editor="Ruiz-Shulcloper, Jos{\'e}
and Kropatsch, Walter G.",
title="Supervised Isomap with Dissimilarity Measures in Embedding Learning",
booktitle="Progress in Pattern Recognition, Image Analysis and Applications",
year="2008",
publisher="Springer",
address="Berlin, Heidelberg",
pages="389--396",
abstract="In this paper we propose a supervised version of the Isomap algorithm by incorporating class label information into a dissimilarity matrix in a financial analysis setting. On the credible assumption that corporates financial status lie on a low dimensional manifold, nonlinear dimensionality reduction based on manifold learning techniques has strong potential for bankruptcy analysis in financial applications. We apply the method to a real data set of distressed and healthy companies for proper geometric tunning of similarity cases. We show that the accuracy of the proposed approach is comparable to the state-of-the-art Support Vector Machines (SVM) and Relevance Vector Machines (RVM) despite the fewer dimensions used resulting from embedding learning.",
isbn="978-3-540-85920-8",
url = {https://doi.org/10.1007/978-3-540-85920-8\-48}
}


@article{ZHANG2009eslle,
    title = "Enhanced supervised locally linear embedding",
    journal = "Pattern Recognit. Lett",
    volume = "30",
    number = "13",
    pages = "1208 - 1218",
    year = "2009",
    doi = "",
    url = "https://doi.org/10.1016/j.patrec.2009.05.011",
    author = "S. Zhang",
    keywords = "Dimensionality reduction, Supervised locally linear embedding, Face recognition",
    abstract = "In this paper, a new nonlinear dimensionality reduction algorithm, called enhanced supervised locally linear embedding (ESLLE), is proposed. The ESLLE method attempts to make the interclass dissimilarity definitely larger than the intraclass dissimilarity in an effort to strengthen the discriminating power and generalization ability of embedded data representation. Simulation studies on artificial manifold data demonstrate that ESLLE can give better embedding results in dimensionality reduction and is more robust to noise in comparison with the original supervised LLE (SLLE). Experimental results on extended Yale face database B and CMU PIE face databases demonstrate that ESLLE obtains better performance on face recognition compared with other famous methods such as principal component analysis (PCA), locally linear embedding (LLE) as well as SLLE."
}

@ARTICLE{Jia2019ssnmf,
  author={{Jia}, Y. and {Kwong}, S. and {Hou}, J. and others},
  journal={IEEE Trans. Neural. Netw. Learn. Syst.}, 
  title={Semi-Supervised Non-Negative Matrix Factorization With Dissimilarity and Similarity Regularization}, 
  year={2019},
  volume={},
  number={},
  pages={1-12},
  url={http://doi.org/10.1109/TNNLS.2019.2933223}
}


@inproceedings{goldberber2004nca,
author = {Goldberger, J. and Roweis, S. and Hinton, G. and Salakhutdinov, R.},
title = {Neighbourhood Components Analysis},
year = {2004},
publisher = {MIT Press},
address = {Cambridge, MA, USA},
abstract = {In this paper we propose a novel method for learning a Mahalanobis distance measure to be used in the KNN classification algorithm. The algorithm directly maximizes a stochastic variant of the leave-one-out KNN score on the training set. It can also learn a low-dimensional linear embedding of labeled data that can be used for data visualization and fast classification. Unlike other methods, our classification model is non-parametric, making no assumptions about the shape of the class distributions or the boundaries between them. The performance of the method is demonstrated on several data sets, both for metric learning and linear dimensionality reduction.},
booktitle = {Adv. Neural. Inf. Process. Systs.},
pages = {513–520},
numpages = {8},
location = {Vancouver, British Columbia, Canada},
series = {NIPS'04}
}


@book{breiman1984cart,
  added-at = {2020-05-07T22:53:11.000+0200},
  address = {Monterey, CA},
  author = {Breiman, L. and Friedman, J. H. and Olshen, R. A. and Stone, C. J.},
  interhash = {61f3e6d61ba17bb493014bd1c6dfa670},
  intrahash = {7f293aa2bdfd10960ef36928f2795f1d},
  keywords = {ma treelearning},
  publisher = {Wadsworth and Brooks},
  serial = {bre84a},
  timestamp = {2020-05-07T22:53:11.000+0200},
  title = {Classification and Regression Trees},
  year = 1984,
  url = {https://doi.org/10.1201/9781315139470}
}



@inproceedings{sklearn_api,
  author    = {L. Buitinck and G. Louppe and M. Blondel and others},
  title     = {{API} design for machine learning software: experiences from the scikit-learn
               project},
  booktitle = {ECML PKDD Workshop: Languages for Data Mining and Machine Learning},
  year      = {2013},
  pages = {108--122},
}

@Article{Chang2013rnaseq,
author={Chang, K.
and Creighton, C. J.
and Davis, C.
and others},
title={The Cancer Genome Atlas Pan-Cancer analysis project},
journal={Nat. Genet.},
year={2013},
month={Oct},
day={01},
volume={45},
number={10},
pages={1113-1120},
abstract={Current clinical practice is organized according to tissue or organ of origin of tumors. Now, The Cancer Genome Atlas (TCGA) Research Network has started to identify genomic and other molecular commonalities among a dozen different types of cancer. Emerging similarities and contrasts will form the basis for targeted therapies of the future and for repurposing existing therapies by molecular rather than histological similarities of the diseases.},
issn={1546-1718},
doi={10.1038/ng.2764},
url={https://doi.org/10.1038/ng.2764}
}


@TECHREPORT{vangumalli2019kmedoids,
title = {Clustering, Forecasting and Cluster Forecasting: using k-medoids, k-{NN}s and random forests for cluster selection},
author = {Vangumalli, D. R. and Nikolopoulos, K. and Litsiou, K.},
year = {2019},
institution = {Bangor Business School, Prifysgol Bangor University (Cymru / Wales)},
type = {Working Papers},
number = {19016},
abstract = {Data analysts when facing a forecasting task involving a large number of time series, they regularly employ one of the following two methodological approaches: either select a single forecasting method for the entire dataset (aggregate selection), or use the best forecasting method for each time series (individual selection). There is evidence in the predictive analytics literature that the former is more robust than the latter, as in individual selection you tend to overfit models to the data. A third approach is to firstly identify homogeneous clusters within the dataset, and then select a single forecasting method for each cluster (cluster selection). This research examines the performance of three well-celebrated machine learning clustering methods: k-medoids, k-NN and random forests. We then forecast every cluster with the best possible method, and the performance is compared to that of aggregate selection. The aforementioned methods are very often used for classification tasks, but since in our case there is no set of predefined classes, the methods are used for pure clustering. The evaluation is performed in the 645 yearly series of the M3 competition. The empirical evidence suggests that: a) random forests provide the best clusters for the sequential forecasting task, and b) cluster selection has the potential to outperform aggregate selection.},
keywords = {Clustering; k-medoids; Nearest Neighbors; Random Forests; Forecasting;},
url = {https://doi.org/10.1080/01969722.2021.1902049}
}


@Article{Alhusain2017RFclue,
author={Alhusain, L.
and Hafez, A. M.},
title={Cluster ensemble based on Random Forests for genetic data},
journal={BioData Min.},
year={2017},
month={Dec},
day={15},
volume={10},
number={1},
pages={37},
abstract={Clustering plays a crucial role in several application domains, such as bioinformatics. In bioinformatics, clustering has been extensively used as an approach for detecting interesting patterns in genetic data. One application is population structure analysis, which aims to group individuals into subpopulations based on shared genetic variations, such as single nucleotide polymorphisms. Advances in DNA sequencing technology have facilitated the obtainment of genetic datasets with exceptional sizes. Genetic data usually contain hundreds of thousands of genetic markers genotyped for thousands of individuals, making an efficient means for handling such data desirable.},
issn={1756-0381},
doi={10.1186/s13040-017-0156-2},
url={https://doi.org/10.1186/s13040-017-0156-2}
}

@article{ALDRICH2010Fault,
title = {Fault detection and diagnosis with random forest feature extraction and variable importance methods},
journal = {IFAC Proceedings Volumes},
volume = {43},
number = {9},
pages = {79-86},
year = {2010},
note = {13th IFAC Symposium on Automation in Mining, Mineral and Metal Processing},
issn = {1474-6670},
doi = {10.3182/20100802-3-ZA-2014.00020},
url = {https://doi.org/10.3182/20100802-3-ZA-2014.00020},
author = {C. Aldrich and L. Auret},
keywords = {Random forest models, feature extraction, variable importance, fault diagnosis, multivariate statistical process control},
abstract = {The ever-present drive to safer, more cost-effective and cleaner processes motivates the exploration of a variety of process monitoring methods. In the domain of data-driven approaches, random forest models present a nonlinear framework. Random forest models consist of ensembles of classification and regression trees in which the model response is determined by voting committees of independent binary decision trees. Data-driven approaches to fault diagnosis often involve summarizing potentially large numbers of process variables in lower dimensional diagnostic sequences. Random forest feature extraction allows for the monitoring of process in feature and residual spaces, while random forest variable importance measures can potentially be used to identify process variables contribution to fault conditions. In this study, a framework for diagnosing steady state faults with random forests is proposed and demonstrated with a simple nonlinear system and the benchmark Tennessee Eastman process.}
}


@article{slot2022turbine,
author = {M. S. Nielsen and V. Rohde},
title = {A surrogate model for estimating extreme tower loads on wind turbines based on random forest proximities},
journal = {J. Appl. Stat.},
volume = {49},
number = {2},
pages = {485-497},
year  = {2022},
publisher = {Taylor & Francis},
doi = {10.1080/02664763.2020.1815675},
URL = {https://doi.org/10.1080/02664763.2020.1815675},
eprint = {https://doi.org/10.1080/02664763.2020.1815675}
}


@article{resende2019detsystems,
author = {Resende, P. A. A. and Drummond, A. C.},
title = {A Survey of Random Forest Based Methods for Intrusion Detection Systems},
year = {2018},
issue_date = {May 2019},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {51},
number = {3},
issn = {0360-0300},
url = {https://doi.org/10.1145/3178582},
doi = {10.1145/3178582},
abstract = {Over the past decades, researchers have been proposing different Intrusion Detection approaches to deal with the increasing number and complexity of threats for computer systems. In this context, Random Forest models have been providing a notable performance on their applications in the realm of the behaviour-based Intrusion Detection Systems. Specificities of the Random Forest model are used to provide classification, feature selection, and proximity metrics. This work provides a comprehensive review of the general basic concepts related to Intrusion Detection Systems, including taxonomies, attacks, data collection, modelling, evaluation metrics, and commonly used methods. It also provides a survey of Random Forest based methods applied in this context, considering the particularities involved in these models. Finally, some open questions and challenges are posed combined with possible directions to deal with them, which may guide future works on the area.},
journal = {ACM Comput. Surv.},
month = {may},
articleno = {48},
numpages = {36},
keywords = {Random Forest methods, Machine Learning, behavioural methods, anomaly detection, Intrusion Detection Systems}
}

@article{Feng2020survival,
  title={Random Forest (RF) Kernel for Regression, Classification and Survival},
  author={D. Feng and R. Baumgartner},
  journal={ArXiv},
  year={2020},
  volume={abs/2009.00089},
  url = {https://arxiv.org/abs/2009.00089}
}

@article{Hinton2015DistillingTK,
  title={Distilling the Knowledge in a Neural Network},
  author={G. E. Hinton and O. Vinyals and J. Dean},
  journal={ArXiv},
  year={2015},
  volume={abs/1503.02531},
  url = {https://arxiv.org/abs/1503.02531}
}

@Article{Amir2013visne,
author={Amir, E. D.
and Davis, K. L.
and Tadmor, M. D.
and Simonds, E. F.
and others},
title={viSNE enables visualization of high dimensional single-cell data and reveals phenotypic heterogeneity of leukemia},
journal={Nat. Biotechnol.},
year={2013},
month={Jun},
day={01},
volume={31},
number={6},
pages={545-552},
abstract={A new tool to visualize high-dimensional single-cell data, when integrated with mass cytometry, reveals phenotypic heterogeneity of human leukemia.},
issn={1546-1696},
doi={10.1038/nbt.2594},
url={https://doi.org/10.1038/nbt.2594}
}

@article{rowies2000lle,
author = {S. T. Roweis  and L. K. Saul },
title = {Nonlinear Dimensionality Reduction by Locally Linear Embedding},
journal = {Science},
volume = {290},
number = {5500},
pages = {2323-2326},
year = {2000},
doi = {10.1126/science.290.5500.2323},
URL = {https://www.science.org/doi/abs/10.1126/science.290.5500.2323},
eprint = {https://www.science.org/doi/pdf/10.1126/science.290.5500.2323},
abstract = {Many areas of science depend on exploratory data analysis and visualization. The need to analyze large amounts of multivariate data raises the fundamental problem of dimensionality reduction: how to discover compact representations of high-dimensional data. Here, we introduce locally linear embedding (LLE), an unsupervised learning algorithm that computes low-dimensional, neighborhood-preserving embeddings of high-dimensional inputs. Unlike clustering methods for local dimensionality reduction, LLE maps its inputs into a single global coordinate system of lower dimensionality, and its optimizations do not involve local minima. By exploiting the local symmetries of linear reconstructions, LLE is able to learn the global structure of nonlinear manifolds, such as those generated by images of faces or documents of text.}}

@inproceedings{belkin2001laplacian,
author = {Belkin, M. and Niyogi, P.},
title = {Laplacian Eigenmaps and Spectral Techniques for Embedding and Clustering},
year = {2001},
publisher = {MIT Press},
address = {Cambridge, MA, USA},
abstract = {Drawing on the correspondence between the graph Laplacian, the Laplace-Beltrami operator on a manifold, and the connections to the heat equation, we propose a geometrically motivated algorithm for constructing a representation for data sampled from a low dimensional manifold embedded in a higher dimensional space. The algorithm provides a computationally efficient approach to nonlinear dimensionality reduction that has locality preserving properties and a natural connection to clustering. Several applications are considered.},
booktitle = {Proceedings of the 14th International Conference on Neural Information Processing Systems: Natural and Synthetic},
pages = {585–591},
numpages = {7},
location = {Vancouver, British Columbia, Canada},
series = {NIPS'01}
}

 @article{Chao2019supdimred, title={Recent Advances in Supervised Dimension Reduction: A Survey}, volume={1}, ISSN={2504-4990}, url={http://dx.doi.org/10.3390/make1010020}, DOI={10.3390/make1010020}, number={1}, journal={Mach. Learn. Knowl. Extr.}, publisher={MDPI AG}, author={Chao, G. and Luo, Y. and Ding, W.}, year={2019}, month={Jan}, pages={341–358}
}

@ARTICLE{Horton1996ecoli,
  title    = "A probabilistic classification system for predicting the cellular
              localization sites of proteins",
  author   = "Horton, P and Nakai, K",
  abstract = "We have defined a simple model of classification which combines
              human provided expert knowledge with probabilistic reasoning. We
              have developed software to implement this model and have applied
              it to the problem of classifying proteins into their various
              cellular localization sites based on their amino acid sequences.
              Since our system requires no hand tuning to learn training data,
              we can now evaluate the prediction accuracy of protein
              localization sites by a more objective cross-validation method
              than earlier studies using production rule type expert systems.
              336 E. coli proteins were classified into 8 classes with an
              accuracy of 81\% while 1484 yeast proteins were classified into
              10 classes with an accuracy of 55\%. Additionally we report
              empirical results using three different strategies for handling
              continuously valued variables in our probabilistic reasoning
              system.",
  journal  = "Proc. Int. Conf. Intell. Syst. Mol. Biol.",
  volume   =  4,
  pages    = "109--115",
  year     =  1996,
  address  = "United States",
  language = "en"
}

@article{coifman2006dm,
title = {Diffusion maps},
journal = {Appl. Comput. Harmon. Anal.},
volume = {21},
number = {1},
pages = {5-30},
year = {2006},
note = {Special Issue: Diffusion Maps and Wavelets},
issn = {1063-5203},
doi = {10.1016/j.acha.2006.04.006},
url = {https://doi.org/10.1016/j.acha.2006.04.006},
author = {R. R. Coifman and S. Lafon},
keywords = {Diffusion processes, Diffusion metric, Manifold learning, Dimensionality reduction, Eigenmaps, Graph Laplacian},
abstract = {In this paper, we provide a framework based upon diffusion processes for finding meaningful geometric descriptions of data sets. We show that eigenfunctions of Markov matrices can be used to construct coordinates called diffusion maps that generate efficient representations of complex geometric structures. The associated family of diffusion distances, obtained by iterating the Markov matrix, defines multiscale geometries that prove to be useful in the context of data parametrization and dimensionality reduction. The proposed framework relates the spectral properties of Markov processes to their geometric counterparts and it unifies ideas arising in a variety of contexts such as machine learning, spectral graph theory and eigenmap methods.}
}


@article{bair2006spc,
author = {E. Bair and T. Hastie and D. Paul and R. Tibshirani},
title = {Prediction by Supervised Principal Components},
journal = {J. Am. Stat. Assoc.},
volume = {101},
number = {473},
pages = {119-137},
year  = {2006},
publisher = {Taylor & Francis},
doi = {10.1198/016214505000000628},

URL = {https://doi.org/10.1198/016214505000000628},
eprint = {https://doi.org/10.1198/016214505000000628}
}

@inproceedings{yu2006spca,
author = {Yu, S. and Yu, K. and Tresp, V. and Kriegel, H. and Wu, M.},
title = {Supervised Probabilistic Principal Component Analysis},
year = {2006},
isbn = {1595933395},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/1150402.1150454},
doi = {10.1145/1150402.1150454},
abstract = {Principal component analysis (PCA) has been extensively applied in data mining, pattern recognition and information retrieval for unsupervised dimensionality reduction. When labels of data are available, e.g., in a classification or regression task, PCA is however not able to use this information. The problem is more interesting if only part of the input data are labeled, i.e., in a semi-supervised setting. In this paper we propose a supervised PCA model called SPPCA and a semi-supervised PCA model called S2PPCA, both of which are extensions of a probabilistic PCA model. The proposed models are able to incorporate the label information into the projection phase, and can naturally handle multiple outputs (i.e., in multi-task learning problems). We derive an efficient EM learning algorithm for both models, and also provide theoretical justifications of the model behaviors. SPPCA and S2PPCA are compared with other supervised projection methods on various learning tasks, and show not only promising performance but also good scalability.},
booktitle = {Proc. ACM SIGKDD Int. Conf. Knowl. Discov. Data Min.},
pages = {464–473},
numpages = {10},
keywords = {dimensionality reduction, supervised projection, principal component analysis, semi-supervised projection},
location = {Philadelphia, PA, USA},
series = {KDD '06}
}


@Article{Vogelstein2021lol,
author={Vogelstein, J. T.
and Bridgeford, E. W.
and Tang, M.
and Zheng, D.
and others},
title={Supervised dimensionality reduction for big data},
journal={Nat. Commun.},
year={2021},
month={May},
day={17},
volume={12},
number={1},
pages={2872},
abstract={To solve key biomedical problems, experimentalists now routinely measure millions or billions of features (dimensions) per sample, with the hope that data science techniques will be able to build accurate data-driven inferences. Because sample sizes are typically orders of magnitude smaller than the dimensionality of these data, valid inferences require finding a low-dimensional representation that preserves the discriminating information (e.g., whether the individual suffers from a particular disease). There is a lack of interpretable supervised dimensionality reduction methods that scale to millions of dimensions with strong statistical theoretical guarantees. We introduce an approach to extending principal components analysis by incorporating class-conditional moment estimates into the low-dimensional projection. The simplest version, Linear Optimal Low-rank projection, incorporates the class-conditional means. We prove, and substantiate with both synthetic and real data benchmarks, that Linear Optimal Low-Rank Projection and its generalizations lead to improved data representations for subsequent classification, while maintaining computational efficiency and scalability. Using multiple brain imaging datasets consisting of more than 150 million features, and several genomics datasets with more than 500,000 features, Linear Optimal Low-Rank Projection outperforms other scalable linear dimensionality reduction techniques in terms of accuracy, while only requiring a few minutes on a standard desktop computer.},
issn={2041-1723},
doi={10.1038/s41467-021-23102-2},
url={https://doi.org/10.1038/s41467-021-23102-2}
}

@Article{Lee1999,
    author={Lee, D.D.
    and Seung, H. S.},
    title={Learning the parts of objects by non-negative matrix factorization},
    journal={Nature},
    year={1999},
    month={Oct},
    day={01},
    volume={401},
    number={6755},
    pages={788-791},
    url = {https://doi.org/10.1038/44565}
}

@article{BARSHAN2011spcav,
title = {Supervised principal component analysis: Visualization, classification and regression on subspaces and submanifolds},
journal = {Pattern Recognit.},
volume = {44},
number = {7},
pages = {1357-1371},
year = {2011},
issn = {0031-3203},
doi = {10.1016/j.patcog.2010.12.015},
url = {https://doi.org/10.1016/j.patcog.2010.12.015},
author = {Elnaz Barshan and Ali Ghodsi and Zohreh Azimifar and Mansoor {Zolghadri Jahromi}},
keywords = {Dimensionality reduction, Principal component analysis (PCA), Kernel methods, Supervised learning, Visualization, Classification, Regression},
abstract = {We propose “supervised principal component analysis (supervised PCA)”, a generalization of PCA that is uniquely effective for regression and classification problems with high-dimensional input data. It works by estimating a sequence of principal components that have maximal dependence on the response variable. The proposed supervised PCA is solvable in closed-form, and has a dual formulation that significantly reduces the computational complexity of problems in which the number of predictors greatly exceeds the number of observations (such as DNA microarray experiments). Furthermore, we show how the algorithm can be kernelized, which makes it applicable to non-linear dimensionality reduction tasks. Experimental results on various visualization, classification and regression problems show significant improvement over other supervised approaches both in accuracy and computational efficiency.}
}


 @article{Tsuge2001,
  title={Dimensionality reduction using non-negative matrix factorization for information retrieval},
  author={Satoru Tsuge and Masami Shishibori and Shingo Kuroiwa and Kenji Kita},
  journal={2001 IEEE International Conference on Systems, Man and Cybernetics. e-Systems and e-Man for Cybernetics in Cyberspace (Cat.No.01CH37236)},
  year={2001},
  volume={2},
  pages={960-965 vol.2},
  url = {http://doi.org/10.1109/ICSMC.2001.973042}
}

 @ARTICLE{Liu2012,
  author={ {Liu}, H. and  {Zhaohui}, W. and  {Xuelong}, L. and others},
  journal={IEEE Trans. Pattern Anal. Mach. Intell.}, 
  title={Constrained Nonnegative Matrix Factorization for Image Representation}, 
  year={2012},
  volume={34},
  number={7},
  pages={1299-1311},
  url = {https://doi.org/10.1007/s11277-018-5325-1}
}

@ARTICLE{Li2018,
  author={Z. {Li} and J. {Tang} and X. {He}},
  journal={IEEE Trans. Neural Netw. Learn. Syst}, 
  title={Robust Structured Nonnegative Matrix Factorization for Image Representation}, 
  year={2018},
  volume={29},
  number={5},
  pages={1947-1960},
  url = {http://doi.org/10.1109/TNNLS.2017.2691725}
}

@ARTICLE{Zhang2016,
  author={X. {Zhang} and L. {Zong} and X. {Liu} and J. {Luo}},
  journal={IEEE Trans. Neural. Netw. Learn. Syst.}, 
  title={Constrained Clustering With Nonnegative Matrix Factorization}, 
  year={2016},
  volume={27},
  number={7},
  pages={1514-1526},
}

@article{Liu2008,
title = "Reducing microarray data via nonnegative matrix factorization for visualization and clustering analysis",
journal = "J. Biomed. Inform.",
volume = "41",
number = "4",
pages = "602 - 606",
year = "2008",
doi = "10.1016/j.jbi.2007.12.003",
url = "https://doi.org/10.1016/j.jbi.2007.12.003",
author = "W. Liu and K. Yuan and D. Ye",
keywords = "Microarray data, Nonnegative Matrix Factorization, Principal component analysis, Visualization, Clustering analysis",
abstract = "In microarray data analysis, each gene expression sample has thousands of genes and reducing such high dimensionality is useful for both visualization and further clustering of samples. Traditional principal component analysis (PCA) is a commonly used method which has problems. Nonnegative Matrix Factorization (NMF) is a new dimension reduction method. In this paper we compare NMF and PCA for dimension reduction. The reduced data is used for visualization, and clustering analysis via k-means on 11 real gene expression datasets. Before the clustering analysis, we apply NMF and PCA for reduction in visualization. The results on one leukemia dataset show that NMF can discover natural clusters and clearly detect one mislabeled sample while PCA cannot. For clustering analysis via k-means, NMF most typically outperforms PCA. Our results demonstrate the superiority of NMF over PCA in reducing microarray data."
}

@article{tapson2005,
title = "PLANT DATA VISUALIZATION USING NON-NEGATIVE MATRIX FACTORIZATION",
journal = "IFAC",
volume = "38",
number = "1",
pages = "73 - 78",
year = "2005",
issn = "1474-6670",
doi = "10.3182/20050703-6-CZ-1902.01814",
url = "https://doi.org/10.3182/20050703-6-CZ-1902.01814",
author = "J. Tapson and J.R. Greene"
}

@article{Babaee2016ImmersiveVO,
  title={Immersive visualization of visual data using nonnegative matrix factorization},
  author={M. Babaee and S. Tsoukalas and G. Rigoll and M. Datcu},
  journal={Neurocomputing},
  year={2016},
  volume={173},
  pages={245-255},
  url = {https://doi.org/10.1016/j.neucom.2015.03.121}
}

  
  @article{Cai2008,
  title={Non-negative Matrix Factorization on Manifold},
  author={Deng Cai and Xiaofei He and Xiaoyun Wu and Jiawei Han},
  journal={2008 Eighth IEEE International Conference on Data Mining},
  year={2008},
  pages={63-72},
  url = {https://doi.org/10.1007/s11063-019-10111-y}
}
  
 @inproceedings{vlachos2002,
author = {Vlachos, M. and Domeniconi, C. and Gunopulos, D. and Kollios, G. and others},
title = {Non-Linear Dimensionality Reduction Techniques for Classification and Visualization},
year = {2002},
isbn = {158113567X},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/775047.775143},
doi = {10.1145/775047.775143},
abstract = {In this paper we address the issue of using local embeddings for data visualization in two and three dimensions, and for classification. We advocate their use on the basis that they provide an efficient mapping procedure from the original dimension of the data, to a lower intrinsic dimension. We depict how they can accurately capture the user's perception of similarity in high-dimensional data for visualization purposes. Moreover, we exploit the low-dimensional mapping provided by these embeddings, to develop new classification techniques, and we show experimentally that the classification accuracy is comparable (albeit using fewer dimensions) to a number of other classification procedures.},
booktitle = {Proceedings of the Eighth ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
pages = {645–651},
numpages = {7},
location = {Edmonton, Alberta, Canada},
series = {KDD '02}
}


@InProceedings{ridder2003,
author="de Ridder, Dick
and Kouropteva, Olga
and Okun, Oleg
and Pietik{\"a}inen, Matti
and Duin, Robert P. W.",
editor="Kaynak, Okyay
and Alpaydin, Ethem
and Oja, Erkki
and Xu, Lei",
title="Supervised Locally Linear Embedding",
booktitle="Artificial Neural Networks and Neural Information Processing --- ICANN/ICONIP 2003",
year="2003",
publisher="Springer",
address="Berlin, Heidelberg",
pages="333--341",
abstract="Locally linear embedding (LLE) is a recently proposed method for unsupervised nonlinear dimensionality reduction. It has a number of attractive features: it does not require an iterative algorithm, and just a few parameters need to be set. Two extensions of LLE to supervised feature extraction were independently proposed by the authors of this paper. Here, both methods are unified in a common framework and applied to a number of benchmark data sets. Results show that they perform very well on high-dimensional data which exhibits a manifold structure.",
isbn="978-3-540-44989-8",
url = {https://doi.org/10.1007/3-540-44989-2-40}
}




@incollection{polito2002,
    title = {Grouping and dimensionality reduction by locally linear embedding},
    author = {M. Polito and Perona, P.},
    booktitle = {NeurIPS},
    editor = {T. G. Dietterich and S. Becker and Z. Ghahramani},
    pages = {1255--1262},
    year = {2002},
    publisher = {MIT Press},
    url = {}
}


@article{anderson1936iris,
 ISSN = {00266493},
 URL = {https://doi.org/10.2307/2394164},
 author = {Edgar Anderson},
 journal = {Annals of the Missouri Botanical Garden},
 number = {3},
 pages = {457--509},
 publisher = {Missouri Botanical Garden Press},
 title = {The Species Problem in Iris},
 urldate = {2022-07-29},
 volume = {23},
 year = {1936}
}




@article{ZHANG2020221labelfree,
title = {Label-free discrimination and quantitative analysis of oxidative stress induced cytotoxicity and potential protection of antioxidants using Raman micro-spectroscopy and machine learning},
journal = {Anal. Chim. Acta},
volume = {1128},
pages = {221-230},
year = {2020},
issn = {0003-2670},
doi = {10.1016/j.aca.2020.06.074},
url = {https://doi.org/10.1016/j.aca.2020.06.074},
author = {Wei Zhang and Jake S. Rhodes and Ankit Garg and Jon Y. Takemoto and Xiaojun Qi and Sitaram Harihar and Cheng-Wei {Tom Chang} and Kevin R. Moon and Anhong Zhou},
keywords = {Raman spectroscopy, Machine learning, PHATE, Mutual information, Antioxidant}
}


  @article{moon2017mi,
  title={Ensemble estimation of mutual information},
  author={Kevin R. Moon and Kumar Sricharan and Alfred O. Hero},
  journal={2017 IEEE International Symposium on Information Theory (ISIT)},
  year={2017},
  pages={3030-3034},
  doi={10.1109/ISIT.2017.8007086}
  
}
  
 @article{ALIKHAN2022salinity,
title = {Application of random forest for modelling of surface water salinity},
journal = {Ain Shams Engineering Journal},
volume = {13},
number = {4},
pages = {101635},
year = {2022},
issn = {2090-4479},
doi = {10.1016/j.asej.2021.11.004},
url = {https://doi.org/10.1016/j.asej.2021.11.004},
author = {M. {Ali Khan} and M. {Izhar Shah} and M. {Faisal Javed} and M. {Ijaz Khan} and others},
keywords = {Surface water salinity, Electrical conductivity (EC), Total dissolved solids (TDS), Inputs optimization, Random Forest modeling},
abstract = {Modeling surface water quality using artificial intelligence-based models is essential in projecting suitable mitigation measures. However, it remains a challenge and requires further research to enhance the modeling accuracy. For this aim, this article presents a methodology to optimize the modeling inputs and reduce the associated complexity. The proposed approach employs Random Forest for modeling surface water salinity in terms of electrical conductivity (EC) and total dissolved solids (TDS) in the upper Indus River basin, one of the major rivers in Asia. Various water quality parameters measured monthly over a historical 30-year period were utilized in the modeling process. Various statistical indicators were used to evaluate the model performance. Random Forest process is suitable technique to simulate the salinity of surface water bodies, and effective tool in minimizing the modeling complexity and elaborating proper management and mitigation measures.}
}

@article{ZHANG2021clay,
title = {Prediction of undrained shear strength using extreme gradient boosting and random forest based on {B}ayesian optimization},
journal = {Geosci. Front.},
volume = {12},
number = {1},
pages = {469-477},
year = {2021},
issn = {1674-9871},
doi = {10.1016/j.gsf.2020.03.0E07},
url = {https://doi.org/10.1016/j.gsf.2020.03.007},
author = {W. Zhang and C. Wu and H. Zhong and Y. Li and L. Wang},
keywords = {Undrained shear strength, Extreme gradient boosting, Random forest, Bayesian optimization, k-fold CV},
abstract = {Accurate assessment of undrained shear strength (USS) for soft sensitive clays is a great concern in geotechnical engineering practice. This study applies novel data-driven extreme gradient boosting (XGBoost) and random forest (RF) ensemble learning methods for capturing the relationships between the USS and various basic soil parameters. Based on the soil data sets from TC304 database, a general approach is developed to predict the USS of soft clays using the two machine learning methods above, where five feature variables including the preconsolidation stress (PS), vertical effective stress (VES), liquid limit (LL), plastic limit (PL) and natural water content (W) are adopted. To reduce the dependence on the rule of thumb and inefficient brute-force search, the Bayesian optimization method is applied to determine the appropriate model hyper-parameters of both XGBoost and RF. The developed models are comprehensively compared with three comparison machine learning methods and two transformation models with respect to predictive accuracy and robustness under 5-fold cross-validation (CV). It is shown that XGBoost-based and RF-based methods outperform these approaches. Besides, the XGBoost-based model provides feature importance ranks, which makes it a promising tool in the prediction of geotechnical parameters and enhances the interpretability of model.}
}

@article{LIN2021co2,
title = {Analyzing the impact of three-dimensional building structure on {CO}$_2$ emissions based on random forest regression},
journal = {Energy},
volume = {236},
pages = {121502},
year = {2021},
issn = {0360-5442},
doi = {10.1016/j.energy.2021.121502},
url = {https://doi.org/10.1016/j.energy.2021.121502},
author = {J. Lin and S. Lu and X. He and F. Wang},
keywords = {CO emission, Building structure, Energy planning, Urban design, Random forest},
abstract = {Carbon dioxide (CO2) is the primary greenhouse gas that increasingly threatens environmental conditions and public health. In addition to conventional socio-economic mitigation measures, a healthy urban design can substantially contribute to the reduction of CO2 emissions. Nevertheless, previous attempts only concentrated on the impacts of horizontal landscape pattern and spatial structure on CO2 emissions. The relationship between three-dimensional building structure and CO2 emissions remains to be explored. To fill this knowledge gap, our study analyzed which building indicators matter most to CO2 emissions in high-density areas. First, we discovered the linear relationships between CO2 emissions and various potential spatial drivers based on Pearson correlation test. Second, we examined whether the additional consideration of different building-related indicators can better explain the variation in CO2 emissions using random forest regression. These experiments indicated that building coverage ratio, mean building number, spatial congestion degree, and floor area ratio can exert substantial impacts on CO2 emissions in the study area. Building structure is a key factor affecting CO2 emission volumes. For example, our improved model yields a lower root relative squared error (32.53\%) than the benchmark model (34.68\%). This methodological framework, which can be easily applied to any other regions, is expected to provide valuable information for the reduction of CO2 emissions from the perspective of vertical urban planning. Policy-makers should carefully consider the impact of building structure on CO2 emissions at an earlier stage of the healthy urban design.}
}

@article{WANG2021water,
title = {Spatial heterogeneity modeling of water quality based on random forest regression and model interpretation},
journal = {Environ. Res.},
volume = {202},
pages = {111660},
year = {2021},
issn = {0013-9351},
doi = {10.1016/j.envres.2021.111660},
url = {https://doi.org/10.1016/j.envres.2021.111660},
author = {F. Wang and Y. Wang and K. Zhang and M. Hu and others},
keywords = {Water quality assessment, Machine learning, Random forest regression, Driving force analysis, Shapley additive explanations}
}

@article{rhodes2023rfgap,
  author={Rhodes, Jake S. and Cutler, Adele and Moon, Kevin R.},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence}, 
  title={Geometry- and Accuracy-Preserving Random Forest Proximities}, 
  year={2023},
  volume={45},
  number={9},
  pages={10947-10959},
  doi={10.1109/TPAMI.2023.3263774}}



@article{GORMAN198875sonar,
title = {Analysis of hidden units in a layered network trained to classify sonar targets},
journal = {Neural Netw},
volume = {1},
number = {1},
pages = {75-89},
year = {1988},
issn = {0893-6080},
doi = {10.1016/0893-6080(88)90023-8},
url = {https://doi.org/10.1016/0893-6080(88)90023-8},
author = {R.Paul Gorman and Terrence J. Sejnowski},
keywords = {Learning algorithms, Hidden units, Multilayered neural network, Sonar, Signal processing},
abstract = {A neural network learning procedure has been applied to the classification of sonar returns from two undersea targets, a metal cylinder and a similarly shaped rock. Networks with an intermediate layer of hidden processing units achieved a classification accuracy as high as 100\% on a training set of 104 returns. These networks correctly classified up to 90.4\% of 104 test returns not contained in the training set. This performance was better than that of a nearest neighbor classifier, which was 82.7\%, and was close to that of an optimal Bayes classifier. Specific signal features extracted by hidden units in a trained network were identified and related to coding schemes in the pattern of connection strengths between the input and the hidden units. Network performance and classification strategy was comparable to that of trained human listeners.}
}

@techreport{brin1998pagerank,
          number = {1999-66},
           month = {November},
          author = {Lawrence Page and Sergey Brin and Rajeev Motwani and Terry Winograd},
            note = {Previous number = SIDL-WP-1999-0120},
           title = {The PageRank Citation Ranking: Bringing Order to the Web.},
            type = {Technical Report},
       publisher = {Stanford InfoLab},
            year = {1999},
     institution = {Stanford InfoLab},
             url = {http://ilpubs.stanford.edu:8090/422/},
        abstract = {The importance of a Web page is an inherently subjective matter, which depends on the readers interests, knowledge and attitudes. But there is still much that can be said objectively about the relative importance of Web pages. This paper describes PageRank, a mathod for rating Web pages objectively and mechanically, effectively measuring the human interest and attention devoted to them. We compare PageRank to an idealized random Web surfer. We show how to efficiently compute PageRank for large numbers of pages. And, we show how to apply PageRank to search and to user navigation.}
}

  @Article{ishwaran2007randomForestSRC,
    title = {Random Survival Forests for R},
    author = {H. Ishwaran and U.B. Kogalur},
    journal = {R News},
    year = {2007},
    volume = {7},
    number = {2},
    pages = {25--31},
    month = {October},
    url = {https://CRAN.R-project.org/doc/Rnews/},
    pdf = {https://CRAN.R-project.org/doc/Rnews/Rnews-2007-2.pdf},
  }

  @Article{hothorn2006party,
    title = {Survival Ensembles},
    author = {Torsten Hothorn and Peter Buehlmann and Sandrine Dudoit
      and Annette Molinaro and Mark {Van Der Laan}},
    journal = {Biostatistics},
    year = {2006},
    volume = {7},
    number = {3},
    pages = {355--373},
    url = {https://doi.org/10.1093/biostatistics/kxj011}
  }
  
  
@Book{ggplot2,
    author = {Hadley Wickham},
    title = {ggplot2: Elegant Graphics for Data Analysis},
    publisher = {Springer},
    year = {2016},
    address="New York, NY",
    isbn = {978-3-319-24277-4},
    url = {https://doi.org/10.1007/978-0-387-98141-3},
}






@article{pearson1901pca,
    author = {Pearson, Karl},
    title = {LIII. On lines and planes of closest fit to systems of points in space},
    journal = {The London, Edinburgh, and Dublin Philosophical Magazine and Journal of Science},
    volume = {2},
    number = {11},
    pages = {559-572},
    year  = {1901},
    publisher = {Taylor & Francis},
    doi = {10.1080/14786440109462720},
    
    URL = {https://doi.org/10.1080/14786440109462720},
    eprint = {https://doi.org/10.1080/14786440109462720}
}

@article{Chawla2002smote,
author = {Chawla, Nitesh V. and Bowyer, Kevin W. and Hall, Lawrence O. and Kegelmeyer, W. Philip},
title = {{SMOTE}: Synthetic Minority over-Sampling Technique},
year = {2002},
issue_date = {January 2002},
publisher = {AI Access Foundation},
address = {El Segundo, CA, USA},
volume = {16},
number = {1},
issn = {1076-9757},
abstract = {An approach to the construction of classifiers from imbalanced datasets is described. A dataset is imbalanced if the classification categories are not approximately equally represented. Often real-world data sets are predominately composed of "normal" examples with only a small percentage of "abnormal" or "interesting" examples. It is also the case that the cost of misclassifying an abnormal (interesting) example as a normal example is often much higher than the cost of the reverse error. Under-sampling of the majority (normal) class has been proposed as a good means of increasing the sensitivity of a classifier to the minority class. This paper shows that a combination of our method of oversampling the minority (abnormal)cla ss and under-sampling the majority (normal) class can achieve better classifier performance (in ROC space)tha n only under-sampling the majority class. This paper also shows that a combination of our method of over-sampling the minority class and under-sampling the majority class can achieve better classifier performance (in ROC space)t han varying the loss ratios in Ripper or class priors in Naive Bayes. Our method of over-sampling the minority class involves creating synthetic minority class examples. Experiments are performed using C4.5, Ripper and a Naive Bayes classifier. The method is evaluated using the area under the Receiver Operating Characteristic curve (AUC)and the ROC convex hull strategy.},
journal = {J. Artif. Int. Res.},
month = {jun},
pages = {321–357},
numpages = {37}
}


@ARTICLE{ramanchadram2017multimodal,
  author={Ramachandram, Dhanesh and Taylor, Graham W.},
  journal={IEEE Signal Processing Magazine}, 
  title={Deep Multimodal Learning: A Survey on Recent Advances and Trends}, 
  year={2017},
  volume={34},
  number={6},
  pages={96-108},
  doi={10.1109/MSP.2017.2738401},
  url = {http://doi.org/10.1109/MSP.2017.2738401}}
  
  
  
@Manual{rockel2020missMethods,
title = {missMethods: Methods for Missing Data},
author = {Tobias Rockel},
year = {2020},
note = {R package version 0.2.0},
url = {https://CRAN.R-project.org/package=missMethods},
}

@inproceedings{hinton1994autoencoders,
 author = {Hinton, Geoffrey E and Zemel, Richard},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {J. Cowan and G. Tesauro and J. Alspector},
 pages = {},
 publisher = {Morgan-Kaufmann},
 title = {Autoencoders, Minimum Description Length and Helmholtz Free Energy},
 url = {https://proceedings.neurips.cc/paper/1993/file/9e3cfc48eccf81a0d57663e129aef3cb-Paper.pdf},
 volume = {6},
 year = {1993}
}

@ARTICLE{cheng2015stsne,  
    author={Cheng, J. and Liu, H. and Wang, F. and Li,             H. and Zhu, C.},  
    journal={IEEE Transactions on Image Processing},   
    title={Silhouette Analysis for Human Action Recognition Based on Supervised Temporal {t-SNE} and Incremental Learning},   
    year={2015},  
    volume={24},  
    number={10},  
    pages={3203-3217},  
    doi={10.1109/TIP.2015.2441634},
    url = {http://doi.org/10.1109/TIP.2015.2441634}
    }
    
    
@inproceedings{hajderanj2019stsne,
    author = {Hajderanj, L. and Weheliye, I. and Chen, D.},
    title = {A New Supervised {T-SNE} with Dissimilarity Measure for Effective Data Visualization and Classification},
    year = {2019},
    isbn = {9781450361057},
    publisher = {Association for Computing Machinery},
    address = {New York, NY, USA},
    url = {https://doi.org/10.1145/3328833.3328853},
    doi = {10.1145/3328833.3328853},
    abstract = {In this paper, a new version of the Supervised t- Stochastic Neighbor Embedding (S-tSNE) algorithm is proposed which introduces the use of a dissimilarity measure related to class information. The proposed S-tSNE can be applied in any high dimensional dataset for visualization or as a feature extraction for classification problems. In this study, the S-tSNE is applied to three datasets MNIST, Chest x-ray, and SEER Breast Cancer. The two-dimensional data generated by the S-tSNE showed better visualization and an improvement in terms of classification accuracy in comparison to the original t- Stochastic Neighbor Embedding(t-SNE) method. The results from k-nearest neighbors (k-NN) classification model which used the lower dimension space generated by the new S-tSNE method showed more than 20\% improvement on average in accuracy in all the three datasets compared with the t-SNE method. In addition, the classification accuracy using the S-tSNE for feature extraction was even higher than classification accuracy obtained from the original high dimensional data.},
    booktitle = {Proceedings of the 2019 8th International Conference on Software and Information Engineering},
    pages = {232–236},
    numpages = {5},
    keywords = {supervised dimensionality reduction, k-NN classification, dissimilarity measure, High dimensional data, supervised t-SNE},
    location = {Cairo, Egypt},
    series = {ICSIE '19}
    }
    
@article{sainburg2021ssumap,
    author = {Sainburg, Tim and McInnes, Leland and Gentner, Timothy Q.},
    title = "{Parametric UMAP embeddings for representation and semisupervised learning}",
    journal = {Neural Computation},
    volume = {33},
    number = {11},
    pages = {2881-2907},
    year = {2021},
    month = {10},
    abstract = "{UMAP is a nonparametric graph-based dimensionality reduction algorithm using applied Riemannian geometry and algebraic topology to find low-dimensional embeddings of structured data. The UMAP algorithm consists of two steps: (1) computing a graphical representation of a data set (fuzzy simplicial complex) and (2) through stochastic gradient descent, optimizing a low-dimensional embedding of the graph. Here, we extend the second step of UMAP to a parametric optimization over neural network weights, learning a parametric relationship between data and embedding. We first demonstrate that parametric UMAP performs comparably to its nonparametric counterpart while conferring the benefit of a learned parametric mapping (e.g., fast online embeddings for new data). We then explore UMAP as a regularization, constraining the latent distribution of autoencoders, parametrically varying global structure preservation, and improving classifier accuracy for semisupervised learning by capturing structure in unlabeled data.1}",
    issn = {0899-7667},
    doi = {10.1162/neco\-a\-01434},
    url = {https://doi.org/10.1162/neco\-a\-01434},
    eprint = {https://direct.mit.edu/neco/article-pdf/33/11/2881/1966656/neco\-a\-01434.pdf},
}


@article{chun2006seisomap,
  title={Supervised Isomap with Explicit Mapping},
  author={Chun-Guang Li and Jun Guo},
  journal={First International Conference on Innovative Computing, Information and Control - Volume I (ICICIC'06)},
  year={2006},
  volume={3},
  pages={345-348},
  doi={10.1109/ICICIC.2006.530},
  url = {http://doi.org/10.1109/ICICIC.2006.530}
}


@article{fisher1936lda,
    author = {Fisher, R. A.},
    title = {THE USE OF MULTIPLE MEASUREMENTS IN TAXONOMIC PROBLEMS},
    journal = {Annals of Eugenics},
    volume = {7},
    number = {2},
    pages = {179-188},
    doi = {10.1111/j.1469-1809.1936.tb02137.x},
    url = {https://doi.org/10.1111/j.1469-1809.1936.tb02137.x},
    eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1111/j.1469-1809.1936.tb02137.x},
    abstract = {The articles published by the Annals of Eugenics (1925–1954) have been made available online as an historical archive intended for scholarly use. The work of eugenicists was often pervaded by prejudice against racial, ethnic and disabled groups. The online publication of this material for scholarly research purposes is not an endorsement of those views nor a promotion of eugenics in any way.},
    year = {1936}
}

@article {amouzgar2022hsslda,
	author = {Amouzgar, Meelad and Glass, David R. and Baskar, Reema and Averbukh, Inna and Kimmey, Samuel C. and Tsai, Albert G. and Hartmann, Felix J. and Bendall, Sean C.},
	title = {Supervised dimensionality reduction for exploration of single-cell data by Hybrid Subset Selection - Linear Discriminant Analysis},
	elocation-id = {2022.01.06.475279},
	year = {2022},
	doi = {10.1101/2022.01.06.475279},
	publisher = {Cold Spring Harbor Laboratory},
	abstract = {Single-cell technologies generate large, high-dimensional datasets encompassing a diversity of omics. Dimensionality reduction enables visualization of data by representing cells in two-dimensional plots that capture the structure and heterogeneity of the original dataset. Visualizations contribute to human understanding of data and are useful for guiding both quantitative and qualitative analysis of cellular relationships. Existing algorithms are typically unsupervised, utilizing only measured features to generate manifolds, disregarding known biological labels such as cell type or experimental timepoint. Here, we repurpose the classification algorithm, linear discriminant analysis (LDA), for supervised dimensionality reduction of single-cell data. LDA identifies linear combinations of predictors that optimally separate a priori classes, enabling users to tailor visualizations to separate specific aspects of cellular heterogeneity. We implement feature selection by hybrid subset selection (HSS) and demonstrate that this flexible, computationally-efficient approach generates non-stochastic, interpretable axes amenable to diverse biological processes, such as differentiation over time and cell cycle. We benchmark HSS-LDA against several popular dimensionality reduction algorithms and illustrate its utility and versatility for exploration of single-cell mass cytometry, transcriptomics and chromatin accessibility data.Competing Interest StatementThe authors have declared no competing interest.},
	URL = {https://www.biorxiv.org/content/early/2022/01/06/2022.01.06.475279},
	eprint = {https://www.biorxiv.org/content/early/2022/01/06/2022.01.06.475279.full.pdf},
	journal = {bioRxiv}
}

@article{wold2001pls,
title = {PLS-regression: a basic tool of chemometrics},
journal = {Chemometrics and Intelligent Laboratory Systems},
volume = {58},
number = {2},
pages = {109-130},
year = {2001},
note = {PLS Methods},
issn = {0169-7439},
doi = {10.1016/S0169-7439(01)00155-1},
url = {https://doi.org/10.1016/S0169-7439(01)00155-1},
author = {Svante Wold and Michael Sjöström and Lennart Eriksson},
keywords = {PLS, PLSR, Two-block predictive PLS, Latent variables, Multivariate analysis},
abstract = {PLS-regression (PLSR) is the PLS approach in its simplest, and in chemistry and technology, most used form (two-block predictive PLS). PLSR is a method for relating two data matrices, X and Y, by a linear multivariate model, but goes beyond traditional regression in that it models also the structure of X and Y. PLSR derives its usefulness from its ability to analyze data with many, noisy, collinear, and even incomplete variables in both X and Y. PLSR has the desirable property that the precision of the model parameters improves with the increasing number of relevant variables and observations. This article reviews PLSR as it has developed to become a standard tool in chemometrics and used in chemistry and engineering. The underlying model and its assumptions are discussed, and commonly used diagnostics are reviewed together with the interpretation of resulting parameters. Two examples are used as illustrations: First, a Quantitative Structure–Activity Relationship (QSAR)/Quantitative Structure–Property Relationship (QSPR) data set of peptides is used to outline how to develop, interpret and refine a PLSR model. Second, a data set from the manufacturing of recycled paper is analyzed to illustrate time series modelling of process data by means of PLSR and time-lagged X-variables.}
}


@article{mantel1967mantel,
    author = {Mantel, Nathan},
    title = "{The detection of disease clustering and a generalized regression approach}",
    journal = {Cancer Research},
    volume = {27},
    number = {2\-Part\-1},
    pages = {209-220},
    year = {1967},
    month = {02},
    abstract = "{The problem of identifying subtle time-space clustering of disease, as may be occurring in leukemia, is described and reviewed. Published approaches, generally associated with studies of leukemia, not dependent on knowledge of the underlying population for their validity, are directed towards identifying clustering by establishing a relationship between the temporal and the spatial separations for the n(n - 1)/2 possible pairs which can be formed from the n observed cases of disease. Here it is proposed that statistical power can be improved by applying a reciprocal transform to these separations. While a permutational approach can give valid probability levels for any observed association, for reasons of practicability, it is suggested that the observed association be tested relative to its permutational variance. Formulas and computational procedures for doing so are given.While the distance measures between points represent symmetric relationships subject to mathematical and geometric regularities, the variance formula developed is appropriate for arbitrary relationships. Simplified procedures are given for the case of symmetric and skew-symmetric relationships. The general procedure is indicated as being potentially useful in other situations as, for example, the study of interpersonal relationships. Viewing the procedure as a regression approach, the possibility for extending it to nonlinear and multivariate situations is suggested.Other aspects of the problem and of the procedure developed are discussed.Similarly, pure temporal clustering can be identified by a study of incidence rates in periods of widespread epidemics. In point of fact, many epidemics of communicable diseases are somewhat local in nature and so these do actually constitute temporal-spatial clusters. For leukemia and similar diseases in which cases seem to arise substantially at random rather than as clear-cut epidemics, it is necessary to devise sensitive and efficient procedures for detecting any nonrandom component of disease occurrence.Various ingenious procedures which statisticians have developed for the detection of disease clustering are reviewed here. These procedures can be generalized so as to increase their statistical validity and efficiency. The technic to be given below for imparting statistical validity to the procedures already in vogue can be viewed as a generalized form of regression with possible useful application to problems arising in quite different contexts.}",
    issn = {0008-5472},
    eprint = {https://aacrjournals.org/cancerres/article-pdf/27/2\-Part\-1/209/2382183/cr0272p10209.pdf},
}


@article{jiang2009slapeig,
  title={Supervised Laplacian Eigenmaps for Machinery Fault Classification},
  author={Quansheng Jiang and Minping Jia},
  journal={2009 WRI World Congress on Computer Science and Information Engineering},
  year={2009},
  volume={7},
  pages={116-120},
  doi={10.1109/CSIE.2009.765},
  url = {http://doi.org/10.1109/CSIE.2009.765}
}


@InProceedings{ridder2003slle,
author="de Ridder, Dick
and Kouropteva, Olga
and Okun, Oleg
and Pietik{\"a}inen, Matti
and Duin, Robert P. W.",
editor="Kaynak, Okyay
and Alpaydin, Ethem
and Oja, Erkki
and Xu, Lei",
title="Supervised Locally Linear Embedding",
booktitle="Artificial Neural Networks and Neural Information Processing --- ICANN/ICONIP 2003",
year="2003",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="333--341",
abstract="Locally linear embedding (LLE) is a recently proposed method for unsupervised nonlinear dimensionality reduction. It has a number of attractive features: it does not require an iterative algorithm, and just a few parameters need to be set. Two extensions of LLE to supervised feature extraction were independently proposed by the authors of this paper. Here, both methods are unified in a common framework and applied to a number of benchmark data sets. Results show that they perform very well on high-dimensional data which exhibits a manifold structure.",
isbn="978-3-540-44989-8"
}

@ARTICLE{hajderanj2021impactsupman, 
    author={Hajderanj, Laureta and Chen, Daqing and Weheliye, Isakh}, 
    journal={IEEE Access},  
    title={The Impact of Supervised Manifold Learning on Structure Preserving and Classification Error: A Theoretical Study},   
    year={2021},  
    volume={9},  
    number={},  
    pages={43909-43922},  
    doi={10.1109/ACCESS.2021.3066259},
    url = {10.1109/ACCESS.2021.3066259}
}

@Article{Balcan2008simtheory,
    author={Balcan, Maria-Florina
    and Blum, Avrim
    and Srebro, Nathan},
    title={A theory of learning with similarity functions},
    journal={Mach. Learn.},
    year={2008},
    month={Aug},
    day={01},
    volume={72},
    number={1},
    pages={89-112},
    abstract={Kernel functions have become an extremely popular tool in machine learning, with an attractive theory as well. This theory views a kernel as implicitly mapping data points into a possibly very high dimensional space, and describes a kernel function as being good for a given learning problem if data is separable by a large margin in that implicit space. However, while quite elegant, this theory does not necessarily correspond to the intuition of a good kernel as a good measure of similarity, and the underlying margin in the implicit space usually is not apparent in ``natural'' representations of the data. Therefore, it may be difficult for a domain expert to use the theory to help design an appropriate kernel for the learning task at hand. Moreover, the requirement of positive semi-definiteness may rule out the most natural pairwise similarity functions for the given problem domain.},
    issn={1573-0565},
    doi={10.1007/s10994-008-5059-5},
    url={https://doi.org/10.1007/s10994-008-5059-5}
}


@INPROCEEDINGS{duque2019visualizing,
  author={Duque, Andrés F. and Wolf, Guy and Moon, Kevin R.},
  booktitle={2019 IEEE 29th International Workshop on Machine Learning for Signal Processing}, 
  title={Visualizing High Dimensional Dynamical Processes}, 
  year={2019},
  volume={},
  number={},
  pages={1-6},
  address={Pittsburgh, PA},
  doi={10.1109/MLSP.2019.8918875},
  url = {http://doi.org/10.1109/MLSP.2019.8918875}}

  
@article{haghverdi2016diffusion,
  title={Diffusion pseudotime robustly reconstructs lineage branching},
  author={Haghverdi, Laleh and Buettner, Maren and Wolf, F Alexander and Buettner, Florian and Theis, Fabian J},
  journal={Nature Methods},
  volume={13},
  number={10},
  pages={845},
  year={2016},
  publisher={Nature Publishing Group},
  url = {http://doi.org/10.1038/nmeth.3971}
}

@INPROCEEDINGS{bohanec1988cars,
    author = {Marko Bohanec and Vladislav Rajkovič},
    title = {V.: Knowledge Acquisition and Explanation for Multi-Attribute Decision},
    booktitle = {Making, 8 th International Workshop “Expert Systems and Their Applications},
    year = {1988}
}


@article{nadler2006diffusion,
title = {Diffusion maps, spectral clustering and reaction coordinates of dynamical systems},
journal = {Applied and Computational Harmonic Analysis},
volume = {21},
number = {1},
pages = {113-127},
year = {2006},
note = {Special Issue: Diffusion Maps and Wavelets},
issn = {1063-5203},
doi = {10.1016/j.acha.2005.07.004},
url = {https://doi.org/10.1016/j.acha.2005.07.004},
author = {B. Nadler and S. Lafon and R. R. Coifman and I. G. Kevrekidis},
abstract = {A central problem in data analysis is the low dimensional representation of high dimensional data and the concise description of its underlying geometry and density. In the analysis of large scale simulations of complex dynamical systems, where the notion of time evolution comes into play, important problems are the identification of slow variables and dynamically meaningful reaction coordinates that capture the long time evolution of the system. In this paper we provide a unifying view of these apparently different tasks, by considering a family of diffusion maps, defined as the embedding of complex (high dimensional) data onto a low dimensional Euclidean space, via the eigenvectors of suitably defined random walks defined on the given datasets. Assuming that the data is randomly sampled from an underlying general probability distribution p(x)=e−U(x), we show that as the number of samples goes to infinity, the eigenvectors of each diffusion map converge to the eigenfunctions of a corresponding differential operator defined on the support of the probability distribution. Different normalizations of the Markov chain on the graph lead to different limiting differential operators. Specifically, the normalized graph Laplacian leads to a backward Fokker–Planck operator with an underlying potential of 2U(x), best suited for spectral clustering. A different anisotropic normalization of the random walk leads to the backward Fokker–Planck operator with the potential U(x), best suited for the analysis of the long time asymptotics of high dimensional stochastic systems governed by a stochastic differential equation with the same potential U(x). Finally, yet another normalization leads to the eigenfunctions of the Laplace–Beltrami (heat) operator on the manifold in which the data resides, best suited for the analysis of the geometry of the dataset regardless of its possibly non-uniform density.}
}


@Article{Kobak2021tsneglobal,
    author={Kobak, Dmitry
    and Linderman, George C.},
    title={Initialization is critical for preserving global data structure in both {t-SNE} and {UMAP}},
    journal={Nature Biotechnology},
    year={2021},
    month={Feb},
    day={01},
    volume={39},
    number={2},
    pages={156-157},
    issn={1546-1696},
    doi={10.1038/s41587-020-00809-z},
    url={https://doi.org/10.1038/s41587-020-00809-z}
}

@ARTICLE{senanayake2020song,
  author={Senanayake, Damith A. and Wang, Wei and Naik, Shalin H. and Halgamuge, Saman},
  journal={IEEE Transactions on Neural Networks and Learning Systems}, 
  title={Self-Organizing Nebulous Growths for Robust and Incremental Data Visualization}, 
  year={2021},
  volume={32},
  number={10},
  pages={4588-4602},
  doi={10.1109/TNNLS.2020.3023941}}

@article{mcinnes2018umap-software,
  title={UMAP: Uniform Manifold Approximation and Projection},
  author={McInnes, Leland and Healy, John and Saul, Nathaniel and Grossberger, Lukas},
  journal={The Journal of Open Source Software},
  volume={3},
  number={29},
  pages={861},
  year={2018}
}


@misc{naim2019life-expt,
    author = {Mohamed Amine Mairech, Naim1997},
    title = {DataC'EPT : Life expectancy prediction },
    publisher = {Kaggle},
    year = {2019},
    url = {https://kaggle.com/competitions/datacept-life-expectancy-prediction}
}

@inproceedings{
    rhodes2023supervised,
    title={Supervised Manifold Learning via Random Forest Geometry-Preserving Proximities},
    author={Jake Slater Rhodes},
    booktitle={Fourteenth International Conference on Sampling Theory and Applications},
    year={2023},
    url={https://openreview.net/forum?id=t6E4dZjp-e}
}

@misc{rosaler2023enhanced,
      title={Towards Enhanced Local Explainability of Random Forests: a Proximity-Based Approach}, 
      author={Joshua Rosaler and Dhruv Desai and Bhaskarjit Sarmah and Dimitrios Vamvourellis and Deran Onay and Dhagash Mehta and Stefano Pasquali},
      year={2023},
      eprint={2310.12428},
      archivePrefix={arXiv},
      primaryClass={stat.ML}
}

@article{anand2011vne,
  title = {Shannon and von Neumann entropy of random networks with heterogeneous expected degree},
  author = {Anand, Kartik and Bianconi, Ginestra and Severini, Simone},
  journal = {Phys. Rev. E},
  volume = {83},
  issue = {3},
  pages = {036109},
  numpages = {8},
  year = {2011},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.83.036109},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.83.036109}
}


@InProceedings{pierre2012autoencoders,
  title = 	 {Autoencoders, Unsupervised Learning, and Deep Architectures},
  author = 	 {Baldi, Pierre},
  booktitle = 	 {Proceedings of ICML Workshop on Unsupervised and Transfer Learning},
  pages = 	 {37--49},
  year = 	 {2012},
  editor = 	 {Guyon, Isabelle and Dror, Gideon and Lemaire, Vincent and Taylor, Graham and Silver, Daniel},
  volume = 	 {27},
  series = 	 {Proceedings of Machine Learning Research},
  address = 	 {Bellevue, Washington, USA},
  month = 	 {02 Jul},
  publisher =    {PMLR},
  pdf = 	 {http://proceedings.mlr.press/v27/baldi12a/baldi12a.pdf},
  url = 	 {https://proceedings.mlr.press/v27/baldi12a.html},
  abstract = 	 {Autoencoders play a fundamental role in unsupervised learning and in deep architectures for transfer learning and other tasks. In spite of their fundamental role, only linear autoencoders over the real numbers have been solved analytically. Here we present a general mathematical framework for the study of both linear and non-linear autoencoders. The framework allows one to derive an analytical treatment for the most non-linear autoencoder, the Boolean autoencoder. Learning in the Boolean autoencoder is equivalent to a clustering problem that can be solved in polynomial time when the number of clusters is small and becomes NP complete when the number of clusters is large. The framework sheds light on the different kinds of autoencoders, their learning complexity, their horizontal and vertical composability in deep architectures, their critical points, and their fundamental connections to clustering, Hebbian learning, and information theory.}
}

@article{theis2017lossy,
  title={Lossy image compression with compressive autoencoders},
  author={Theis, Lucas and Shi, Wenzhe and Cunningham, Andrew and Husz{\'a}r, Ferenc},
  journal={arXiv preprint arXiv:1703.00395},
  year={2017}
}

@article{romero2017quantum,
  title={Quantum autoencoders for efficient compression of quantum data},
  author={Romero, Jonathan and Olson, Jonathan P and Aspuru-Guzik, Alan},
  journal={Quantum Science and Technology},
  volume={2},
  number={4},
  pages={045001},
  year={2017},
  publisher={IOP Publishing}
}

@misc{titanic2016kaggle,
    author = {Creator: Kaggle},
    title = {Titanic: Machine Learning from Disaster},
    howpublished = {\url{https://www.kaggle.com/c/titanic/data}},
    year = {2016},
    note = {Accessed: 11/13/2023},
}

@article{lecun2010mnist,
    title={MNIST handwritten digit database},
    author={LeCun, Yann and Cortes, Corinna and Burges, CJ},
    journal={AT\&T Labs [Online]. Available: http://yann.lecun.com/exdb/mnist},
    year={2010}
}


@article {Rhodes2023RFPHATE,
	author = {Jake S Rhodes and Adrien Aumon and Sacha Morin and Marc Girard and Catherine Larochelle and Boaz Lahav and Elsa Brunet-Ratnasingham and Wei Zhang and Adele Cutler and Anhong Zhou and Daniel E Kaufmann and Stephanie Zandee and Alexandre Prat and Guy Wolf and Kevin R. Moon},
	title = {Gaining Biological Insights through Supervised Data Visualization},
	elocation-id = {2023.11.22.568384},
	year = {2023},
	doi = {10.1101/2023.11.22.568384},
	publisher = {Cold Spring Harbor Laboratory},
	abstract = {Dimensionality reduction-based data visualization is pivotal in comprehending complex biological data. The most common methods, such as PHATE, t-SNE, and UMAP, are unsupervised and therefore reflect the dominant structure in the data, which may be independent of expert-provided labels. Here we introduce a supervised data visualization method called RF-PHATE, which integrates expert knowledge for further exploration of the data. RF-PHATE leverages random forests to capture intricate feature-label relationships. Extracting information from the forest, RF-PHATE generates low-dimensional visualizations that highlight relevant data relationships while disregarding extraneous features. This approach scales to large datasets and applies to classification and regression. We illustrate RF-PHATE{\textquoteright}s prowess through three case studies. In a multiple sclerosis study using longitudinal clinical and imaging data, RF-PHATE unveils a sub-group of patients with non-benign relapsing-remitting Multiple Sclerosis, demonstrating its aptitude for time-series data. In the context of Raman spectral data, RF-PHATE effectively showcases the impact of antioxidants on diesel exhaust-exposed lung cells, highlighting its proficiency in noisy environments. Furthermore, RF-PHATE aligns established geometric structures with COVID-19 patient outcomes, enriching interpretability in a hierarchical manner.Competing Interest StatementThe authors have declared no competing interest.},
	URL = {https://www.biorxiv.org/content/early/2023/11/23/2023.11.22.568384},
	eprint = {https://www.biorxiv.org/content/early/2023/11/23/2023.11.22.568384.full.pdf},
	journal = {bioRxiv}
}

@article{xiao2017fashion,
  title={Fashion-mnist: a novel image dataset for benchmarking machine learning algorithms},
  author={Xiao, Han and Rasul, Kashif and Vollgraf, Roland},
  journal={arXiv preprint arXiv:1708.07747},
  year={2017}
}

@article{coifman2006geometric,
  title={Geometric harmonics: a novel tool for multiscale out-of-sample extension of empirical functions},
  author={Coifman, Ronald R and Lafon, St{\'e}phane},
  journal={Applied and Computational Harmonic Analysis},
  volume={21},
  number={1},
  pages={31--52},
  year={2006},
  publisher={Elsevier}
}

@article{bengio2003out,
  title={Out-of-sample extensions for lle, isomap, mds, eigenmaps, and spectral clustering},
  author={Bengio, Yoshua and Paiement, Jean-fran{\c{c}}cois and Vincent, Pascal and Delalleau, Olivier and Roux, Nicolas and Ouimet, Marie},
  journal={Advances in neural information processing systems},
  volume={16},
  year={2003}
}
